Extremal combinatorics, iterated pigeonhole arguments, and generalizations of PPP

We study the complexity of computational problems arising from existence theorems in extremal combinatorics. For some of these problems, a solution is guaranteed to exist based on an iterated application of the Pigeonhole Principle. This results in the definition of a new complexity class within TFNP, which we call PLC (for "polynomial long choice"). PLC includes all of PPP, as well as numerous previously unclassified total problems, including search problems related to Ramsey's theorem, the Sunflower theorem, the Erd\H{o}s-Ko-Rado lemma, and K\"onig's lemma. Whether the first two of these four problems are PLC-complete is an important open question which we pursue; in contrast, we show that the latter two are PPP-complete. Finally, we reframe PPP as an optimization problem, and define a hierarchy of such problems related to Tur\'an's theorem.

==> Blockchains.tex <==
\section{Applications to Blockchains}

\subsection{Blockchains: Basic Summary/Algorithm}
\textbf{Note: This section will likely be massively condensed and/or moved to the appendix. It is just for reference for now.}
In this section, we consider how the Long Choice problem can be used as a protocol for building blockchains. Conceptually, a blockchain can be visualized as a sequence of data points which form a ``linked list" data structure: 

\begin{align}
    \text{Block 1} \mapsto \text{Block 2} \mapsto \text{Block 3} \mapsto \dots
\end{align}

Critically, each block will contain some important piece of information; maybe a financial transaction. One question remains: how are the blocks related and why do they form a linked list structure? This interdependence comes from one fact: for $i > 1$, the complete message contained in block $i$ depends on the message contained in block $i-1$. 

This relationship is best illustrated by a concrete example. Suppose we would like to construct a blockchain in which every block contains a finite number (say, $k$) of financial transactions. The maximum number of bits needed to encode these $k$ transactions is $b(k)$, for some polynomial function $b$. Accordingly, we can say that each block contains a total of $n$ bits, for some $n$ which is polynomially larger than $b(k)$. We now define the relationships between blocks in an inductive fashion. 

As a base case, block $1$ contains, as its first $b(k)$ bits, the message describing $k$ financial transactions. The remaining bits are all $0$. Now, suppose all blocks up to block $i$ are defined. Block $i+1$ contains, as its first $b(k)$ bits, a bit string describing its $k$ transactions. The next $c(n)$ bits are a hash of the bit string of block $i$. The remaining $n - c(n) - b(k)$ must extend the first $c(n) + b(k)$ bits of block $i+1$ to solve a computationally intensive puzzle (this puzzle can vary). 

The key point in this definition is that for each block, $i>1$, the entire $n$-bits form the certificate to the computational puzzle, not just the last $n - b(k) - c(n)$ bits. This establishes a strong dependence of block $i+1$'s certificate on block $i$'s overall bitstring. To see why, suppose we have constructed block $i+1$ in a way that satisfies the above definition. If we modify the bit string of block $i$, we likely end up modifying the hash of block $i$'s bitstring. This, in turn modifies the bit string of block $i+1$ (which contains a hash of block $i$). However, after modifying block $i+1$'s string, it may no longer be a valid certificate for the computational puzzle. Therefore, the validity of block $i+1$'s string directly depends on the value of block $i$'s string. 

We now provide some observations about this computationally intensive puzzle. First, it must have a totality property. In particular, regardless of what the first $b(k) + c(n)$ bits are, it must be possible to extend extend these bits with $n - b(k) - c(n)$ so that the entire $n$-bit string forms a certificate to the puzzle of interest. This is necessary, because one may wish to encode messages of any kind in a blockchain. Second, it should be possible to toggle the difficulty of this problem, to allow quicker (or slower) construction of the blockchain. Finally, all certificates should be highly uncorrelated. In other words, given a single certificate, it should be extremely challenging to find a second one. 

\subsection{Long Choice for Blockchain Protocols}
We show how the Long Choice problem can be used to implement a blockchain protocol. Recall that the Long Choice problem is equivalent to a variation of the Long Choice problem in which we fix the first element. In this discussion, we use Long Choice problems with the following in mind: (a) the blockchain miner will want to construct a Long Choice sequence with an initial element of his/her choosing; this initial element will contain the core data of the block (b) each block only contains the first $H$ elements of a valid Long Choice certificate, for some adjustable value $H$; this allows us to toggle the difficulty of the Long Choice problems which miners have to solve. 

We now define the blockchain construction inductively. We begin by defining the functionality of block $1$. We assume, as mentioned above, that each block contains a message of at most $b(k)$ bits. We specify a Long Choice problem instance over the universe of $n$-bit strings, for some predefined $n$ which is larger than $b(k)$. In practice, $n$ can be a large value like 256. In this Long Choice problem instance, the miner wants to construct a certificate in which the first element $a_0$ has a binary encoding has the following properties:

\begin{enumerate}
    \item The first $b(k)$ bits encode the message of interest
    \item The remaining bits are completely randomized.
\end{enumerate}

This is clearly possible because the first element, $a_0$ can be anything (due to the totality of the problem).

A valid string for block $1$ then consists of the first $H$ elements of a Long Choice sequence, in which $a_0$ is the first element. 

We now describe how to construct the next element of this sequence. 

In block $1$, we have a long choice sequence, $a_{1,0}, a_{1, 1}, a_{1,2}, \dots, a_{1, H-1}$. 

Suppose the first $i$ blocks have been established. Then, to construct block $i+1$, our blockchain network samples a Long Choice problem instance (note, it may be possible to reuse the same Long Choice problem instance here across blocks...). 

Next, let $a_0$ denote the first element of block $i$'s Long Choice certificate. The key point is the following: block $i+1$ must contain a sequence $b_0, b_1, \dots, b_{H-1}$ with the property that $a_0 + b_0, a_0 + b_1, \dots, a_{H-1} + b_{H-1}$ form a Long Choice certificate. (Here, $+$ denotes a bit-wise modulo 2 addition operation). Furthermore, $b_0$ must contain the message of interest in block $i+1$. 

We now explain why this construction has desirable properties for a blockchain. First, the Long Choice problem is total: no matter the initial element, we can always find a complete certificate. This must be true of any valid Blockchain protocol. Second, the problem can be made harder by increasing the constant, $H$. Third, consider an adversary who wishes to corrupt this blockchain. Every block of this chain contains a long choice sequence of length $H$, which is a sequence of $H$ $n$-bit strings. In each sequence, the first $n$-bit string contains the information of interest. The adversary will presumably want to corrupt this string. Consider the blocks $i$ and $i+1$:

\begin{align}
    \text{block i}: a_0 \mapsto a_1 \mapsto a_2 \dots \mapsto a_{H-1}\\
    \text{block i+1}: a_0+b_0 \mapsto a_0+b_1 \mapsto a_0+b2 \dots \mapsto a_0 + b_{H-1}
\end{align}
It is clear that by changing even one bit of $a_0$, the adversary will change every single element of block $i+1$. Therefore, it seems extremely likely that they will invalidate the certificates not only for block $i$ but also for block $i+1$ (and all subsequent blocks). Thus, to corrupt block $i$, the adversary likely has to re-solve a Long Choice problem for block $i$ and \textit{all subsequent blocks}. In a proof of work scenario where the longest blockchain is considered legitimate, the adversary can only succeed here if they have the majority of the computational resources in the network. 

The following questions arise: 
\begin{enumerate}
    \item What advantages does this construction have over the SHA-256 based problems used in the bitcoin proof-of-work mining algorithm?
    \item Unlike the current bitcoin mining protocol which uses hashing, the above protocol assumes a fixed message length (whereas SHA-type hashing can rely on variable message length). In what ways might this be an issue?
    \item Do we need to sample a new Long Choice problem for each block? This can be easily done: every day, the network can require that a specific Long Choice problem instance (sampled from a average-case-hard family of Long Choice problems) be used.
    \item Because PPP is contained in Long Choice, every hard family of PWPP problems can, in turn, give rise to a family of hard Long Choice problem instances. This means we can use any PWPP hardness result to generate hard Long Choice instances. Is this particularly useful?
    \item We can take the above point further: we can construct a Long Choice problem instance using all PPP hardness results. 
    \item Beyond blockchains for finance, what other applications exist for Long Choice? It seems that Long Choice can be made into a protocol of some sort (reminiscent of IP or AM). For example, a user can specify a first element $a_0$ and a recevier can provide a predicate function $P_0$ (as in Long Choice). Once the user specifies an element $a_1$, the receiver then provides the next predicaet function. Note that in this protocol, there must exist a valid set of choices which the user can make (however hard this is). Can this be useful in other applications such as DDoS protection or spam prevention? 
\end{enumerate}



==> Compactness.tex <==

\section{Finitary Characterizations of Ramsey and Sunflower}

Ramsey and Sunflower are two combinatorial structures can be characterized by their substructures: 

\begin{theorem}
	A collection, $F$, of distinct sets of size $n$ is a sunflower if and only if for every $s_i, s_j, s_k \in{F}$, $i$, $j$, $k$ form a sunflower of size $3$. 
\end{theorem}
\begin{proof}
	Suppose that $F$ is a sunflower. Then, by definition, any pair of elements has a constant intersection. Thus, any triple of elements of $F$ form a sunflower. 
	Next, suppose that every triple $s_i, s_j, s_k$ form a sunflower. Let $I = s_i \cap s_j$ be the intersection of two of these sets. It suffices to show that for any two sets in $F$, $s_a$ and $s_b$, we have $s_a\cap{s_b} = I$. By our assumption, we know that the triple $s_i, s_a, s_b$ must form a sunflower. We also know that $s_i, s_j, s_a$ must form a sunflower. Thus, $s_i \cap {s_a} = s_i \cap{s_j} = I$. Finally, we have $s_a \cap{s_b} = s_i\cap{s_a} = I$. This completes the proof. 
\end{proof}

\begin{theorem}
	In a graph, a collection of nodes $n_1, \dots, n_i$ form a monochromatic clique if and only if for every $i, j, k \in [i]$, $n_i$, $n_j$, and $n_k$ form a clique. 
\end{theorem}

\begin{proof}
	Suppose that nodes $n_1, \dots, n_i$ form a monochromatic clique. Then, by definition, any pair of nodes has an edge of some fixed color, say, blue. Thus, any triple of elements of $F$ forms a monochromatic clique in which each edge is colored blue. 
	Next, suppose that every triple $n_i, n_j, n_k$ form a monochromatic clique. Let $C = E(n_i, n_j)$ be the color of the edge between $n_i$ and $n_j$. It suffices to show that for any two nodes in $F$, $n_a$ and $n_b$, we have $E(n_a,n_b) = C$. By our assumption, we know that the triple $n_i, n_a, n_b$ must form a monochromatic clique. We also know that $n_i, n_j, n_a$ must form a monochromatic clique. Thus, $E(n_i n_a) = E(n_i,n_j) = C$. Finally, we have $E(n_a,n_b) = E(n_i,n_a)= C$. This completes the proof. 
\end{proof}

We note that Ramsey, Sunflower, and Long Choice all have infinitary and finitary forms; the infinitary forms essentially extent the argument of the finitary problems using the infinite Pigeonhole Principle. \textbf{The discussion from this section raises a significant open question: what other combinatorial structures can be characterized by their finite substructures? }

The theme of compactness also applies to Schur's Theorem, where we have the following result: 

\begin{theorem}
	The infinitary form of Schur's Theorem states that every coloring of the set of positive integers using $r$ colors contains monochromatic $a$, $b$, and $a+b$. This theorem is equivalent to any form of Schur's Theorem (independent of the extremal bound). 
\end{theorem}

\begin{proof}
	First note that if the finitary form is true, then there exists an integer $n$ such that any coloring using $r$ colors which produces a monochromatic $x$, $y$, and $x + y$. Then, for any coloring of the set of positives integers using $r$ colors, we just consider the first $n$ integers. By the finitary theorem, we are done. 
	
	Now, suppose the finitary theorem is false. That is, for every integer $n$, there exists a coloring of the first $n$ numbers such that there is no monochromatic $x$, $y$, and $x + y$. Using the standard compactness argument, can extend these finite colorings to an infinite coloring that does not have the desired monochromatic triples. Thus, we have proved that if the finitary theorem is false, the infinitary theorem is false. Taking the contrapositive of this, we see that the infinitary statement implies the finitary statement. 
\end{proof}




==> Extremal.tex <==
\section{Mantel, Tur\'an, and Bad Colorings}

% At this point, we must ask: what distinguishes Long Choice and PLC from other TFNP search problems from extremal combinatorics? As discussed in this section, perhaps the biggest difference comes from the \textit{number} of distinct valid certificates available in a single problem instance. 

In this section, we introduce a new flavor of problems from extremal combinatorics which generalize PPP. This class of problems is related to Mantel's and Tur\'an's theorem and graph colorings.
Mantel's theorem states that a triangle-free graph with $N$ nodes has at maximum $\lfloor N^2/4 \rfloor$ edges. The maximum is achieved by a complete bipartite graph with equal or almost equal parts (depending on whether $N$ is even or odd).
Tur\'an's theorem answers the generalized question of what is the maximum number of edges in a graph with $N$ nodes that does not contain a $(k+1)$-clique: the maximum is achieved by a complete $k$-partite graph that has equal or almost equal parts  
(see \citep{jukna} for a detailed exposition). 

The same quantities answer the easier question of, what is the maximum number of edges of a $k$-colorable graph on $N$ nodes.
A $k$-colorable graph whose color classes have sizes $x_1, \ldots, x_k$ can have at most $\sum_{i \neq j} x_i x_j$ edges. Since the $x_i$'s are integers that sum to $N$, it can be shown that the maximum is achieved when they are all equal or almost equal.

These theorems induce corresponding total computational problems: Given (succinctly) an exponential graph with more edges than the above bounds of Mantel or Tur\'an, find a triangle or a $(k+1)$-clique respectively.
If we are given in addition a $k$-coloring of the nodes, find an illegally colored edge.
We call these problems respectively {\sc Mantel},
{\sc $k$-Tur\'an} and {\sc Bad $k$-Coloring} 
({\sc Mantel} is just {\sc $2$-Tur\'an}).
We define below formally the problems as TFNP problems.

\begin{defi}[{\sc $k$-Tur\'an}]
   We are given a poly($n$)-sized circuit $E: [ {{k}\choose{2}} (2^n)^2+1] \mapsto [(k 2^n)^2]$, which is supposed to represent a graph with $k 2^n$ nodes
   and ${{k}\choose{2}} (2^n)^2+1$ edges (nodes and indices of edges are encoded by bit-strings of appropriate length as usual); $E$ maps the index of an edge to the two nodes of the edge. The problem is to find either a violation ($E$ is not a valid encoding of the edges of a graph) or a $(k+1)$-clique. Specifically, return one of the following certificates:
   	\begin{enumerate}
 		\item (Error): An index $i$ such that $E(i)$ consists of two identical nodes, or two distinct indices $i,j$ such that $E(i), E(j)$ contain the same two nodes
 		(not necessarily in the same order), or
 		\item ($(k+1)$-clique): ${k+1}\choose{2}$ indices which are mapped by $E$ to the edges of a clique on $k+1$ nodes.
	\end{enumerate}
\end{defi}

\begin{defi}[{\sc Bad $k$-Coloring}]
    We are given a poly($n$)-sized circuit $E: [ {{k}\choose{2}} (2^n)^2+1] \mapsto [(k 2^n)^2]$, which is supposed to represent a graph with $k 2^n$ nodes
   and ${{k}\choose{2}} (2^n)^2+1$ edges and a poly($n$)-sized circuit $C: [k 2^n] \mapsto [k] $ which colors the nodes with $k$ colors. The problem is to find either a violation ($E$ is not a valid encoding of the edges of a graph) or an edge whose nodes have the same color. Specifically, return one of the following certificates:
   	\begin{enumerate}
 		\item (Error): An index $i$ such that $E(i)$ consists of two identical nodes, or two distinct indices $i,j$ such that $E(i), E(j)$ contain the same two nodes
 		(not necessarily in the same order), or
 		\item (Bad edge): An index $i$ such that $E(i) = (a,b)$ and $C(a)=C(b)$.
	\end{enumerate}
\end{defi}

We show the following relations between PPP and these problems
(proofs in the Appendix):

\begin{theorem}
1. PPP reduces to {\sc Bad $2$-Coloring}.\\
2. For all $k \geq 2$, {\sc Bad $k$-Coloring} reduces to {\sc $k$-Tur\'an}. In particular, {\sc Bad $2$-Coloring} reduces to {\sc Mantel}.\\
3. For all $k \geq 2$, {\sc Bad $k$-Coloring} reduces to {\sc Bad $(k+1)$-Coloring}.\\
4. For all $k \geq 2$, {\sc $k$ Tur\'an} reduces to {\sc $(k+1)$-Tur\'an}.
\end{theorem}


Thus, we have a hierarchy of problems on top of PPP.  The Bad Coloring problems can be viewed as instances of the pigeonhole problem 
(there is no iteration here), but the mapping is given indirectly and cannot be easily constructed:
We can view the indices of the edges as the pigeons and the potential legal edges, i.e. all the pairs of differently colored nodes, as the holes. There are more pigeons that holes, so either two pigeons are mapped to the same hole
($E(i), E(j)$ are the same edge for some pair of indices $i,j$)), or some pigeon is not mapped to a hole (for some $i$, $E(i)=(a,a)$ or $E(i)=(a,b)$ with $C(a)=C(b)$; this corresponds to the special 0 value in the PPP problem). The difference with PPP, is that the set of holes (the range of the mapping) is not given a priori explicitly 
as a set of bit-strings (or integers) as in PPP,
but rather it is implied indirectly by the coloring $C$.
As a consequence, even for $k=2$, we cannot compute easily in polynomial time for example the number $h$ of available holes ($h$ is the product of the sizes of the two color classes), and we cannot compute efficiently an index function mapping each legal pair of nodes (pair $(a,b)$ with $C(a) \neq C(b)$) to an index in $[h]$. 
In the Tur\'an problems, there is in addition the complication of optimizing over all partitions (colorings) and of seeking a clique rather than a single edge.

Another example along the same lines is the following  {\sc bad $k$-set coloring} problem; Given (poly($n$)-size circuits specifying) a $k$-coloring $C$ of a set $V$ of $k 2^n$ nodes and a family $F$ of $2^{kn}+1$ $k$-sets over $V$, find a $k$-set in $F$ that is not panchromatic, i.e. two of its elements have the same color, or find two equal sets in $F$. Clearly, the case $k$=1 is the {\sc Collision} problem (which defines PPP). For higher values of $k$, the problems form a hierarchy, where again existence of a certificate is guaranteed by (1) the answer to an optimization problem (what is the maximum number of panchromatic $k$-sets over all $k$-colorings), and (2) the pigeonhole principle, where however the mapping is not given explicitly, but is defined indirectly in an inefficient manner. 

\if{false}
% In this section, we introduce numerous problems from TFNP and argue they are either PPP-complete or PPP-hard. In either case, we take careful note of the fact that these problems' certificates have different properties than those from PLC-complete problems. See \citep{jukna} for a detailed exposition on all of these theorems.

\subsection{Mantel's Theorem}

\begin{theorem}[Mantel's Theorem]
	A triangle-free graph with $n$ nodes has at maximum $\lfloor n^2/4 \rfloor$ edges. 
\end{theorem}

It is well-known that bipartite graphs are triangle-free. To construct a graph with $n^2/4$ edges (where $n$ is even), simply divide the nodes of the graph into two groups of equally-sized groups of $n/2$. Then construct all edges connecting nodes from one group to the other. 


% Of course, given an explicit representation of a graph, it is trivial to decide whether or not there is a triangle. Our algorithm would simply look at every $n\choose {3}$ groupings of $3$ vertices and evaluate whether they form a triangle. The problem seems to be harder, however, if the graph is given implicitly by a circuit. We introduce such a problem, which we call "Mantel", below: 

% \begin{defi}[Problem Statement: Mantel]
% 	Consider a graph, $G$, consisting of $2^n$ vertices. Each vertex is encoded by an $n$-bit string. We are given a circuit, $C$, which implicitly defines a set of $2^{2n-2} + 1$ distinct edges. In particular, 
	
% 	$$C: \{0,1\}^{2n-1} \mapsto (\{0,1\}^{n})^2 $$
	
% 	The circuit $C$ takes, as input, a $2n-1$-bit string, and outputs a pair of $2$ $n$-bit strings. Each of these $n$ bit strings represents a node of the graph $G$. In this sense, if $C(a) = (x,y)$, we mean to say that the vertices of $G$ encoded by bitstrings $x$ and $y$ are connected by an edge. 
% 	We only consider the $2n-1$-bit strings whose decimal representations fall in the range $[0, 2^{2n-2}]$, and we call these bitstrings "indices". Mantel's problem asks for the following: 
	
% 	\begin{enumerate}
% 		\item Invalid edge: Return an index which outputs two identical vertices. In other words, find an index $i$ with $C(i) = (x,x)$ for some $n$-bit string $x$. 
% 		\item Repeated edge: Return $2$ different indices, $i$ and $j$, which describe the same edge. This means both $C(i)$ and $C(j)$ are either $(x,y)$ or $(y,x)$ for some $x,y$. 
% 		\item Triangle: Return $3$ different indices $i$, $j$, $k$, which form the edges of a triangle. In other words, $C(i)$, $C(j)$, $C(k)$ should collectively describe $3$ edges of the form $\{a,b\}$, $\{b,c\}$, and $\{a,c\}$.
% 	\end{enumerate}
% \end{defi}


% There is a straightforward way to show that this problem is a TFNP problem (namely, that every instance has a witness). Consider such a Mantel problem instance. If there is an invalid edge, we are done. If there is a repeated edge, we are done. Suppose there are no repeated edges or invalid edges. Then, every edge is unique and valid. Then, on a graph of $2^n$ vertices, there are $2^{2n-2} + 1$ edges. By Mantel's Theorem, some $3$ vertices must form a triangle. 


% We first remark that Mantel's Theorem is a special case of Turan's Theorem, which answers the more general question: given a graph consisting of $n$ vertices, what is the maximum number of edges the graph can have without containing a $k$-clique? Mantel's Theorem deals with the case of $k = 2$. 

% There is a connection between coloring theorems and Mantel's Theorem. Suppose we are given a graph, $G$, and are asked to color its vertices using two colors (say, blue and red). We first define the notion of $2$-colorability: 

% \begin{defi}[$2$-colorability of a graph]
% 	We say a graph, $G$, is $2$-colorable, if its vertices can be colored using two distinct colors in such a way that no two vertices of the same color are connected by an edge. 
% \end{defi}

% When is a graph $2$-colorable? There is a well-known result that answers this question: 

% \begin{theorem}
% 	A graph $G$ is $2$-colorable if and only if $G$ is bipartite.
% \end{theorem}

% Now, if $G$ has a triangle, it \textit{cannot} be bipartite. To see why, note that no matter how we partition the graph, two nodes from the triangle will end up on the same side, and they will be connected. Therefore, the conditions of Mantel's Theorem guarantee that any coloring of the graph must have a monochromatic edge. That is, for all vertex colorings of the graph $G$, there must exist two monochromatic vertices that are connected. We can define a TFNP problem accordingly. This problem builds on the Mantel problem we have just introduced.

% \begin{defi}[Bad Coloring]
% 	Consider a graph, $G$, consisting of $2^n$ vertices. Each vertex is encoded by an $n$-bit string. We are given a poly(n)-sized circuit, $C$, which implicitly defines a set of $2^{2n-2} + 1$ distinct edges. In particular, 
	
% 	$$C: \{0,1\}^{2n-1} \mapsto (\{0,1\}^{n})^2 $$
	
% 	The circuit $C$ takes, as input, a $(2n-1)$-bit string, and outputs a pair $n$-bit strings. Each of these $n$ bit strings represents a node of the graph $G$. In this sense, if $C(a) = (x,y)$, we mean to say that the vertices of $G$ encoded by bitstrings $x$ and $y$ are connected by an edge. 
% 	We only consider the $(2n-1)$-bit strings whose decimal representations fall in the range $[0, 2^{2n-2}]$.
	
% 	In addition, we are given a coloring function, $F$:
	
% 	$$F: \{0,1\}^{n} \mapsto \{0,1\}$$
% 	$F$ takes as input a single vertex and outputs one of two possible colors, $0$ or $1$. 
	
% 	The Bad Coloring problem asks us to find one of the following: 
% 	\begin{enumerate}
% 		\item Invalid edge: Return an index which outputs two identical vertices. In other words, find an index $i$ with $C(i) = (x,x)$ for some $n$-bit string $x$. 
% 		\item Repeated edge: Return $2$ different indices, $i$ and $j$, which describe the same edge. This means both $C(i)$ and $C(j)$ are either $(x,y)$ or $(y,x)$ for some $x,y$. 
% 		\item Monochromatic Edge: Return a valid edge index $i$ with $C(i) = (a,b)$ such that $F(a) = F(b)$. In other words, find an edge which connects two monochromatic vertices under the coloring $F$. 
% 	\end{enumerate}
% \end{defi}

% We now prove the totality of Bad Coloring. Suppose we are given a Bad Coloring problem instance, which is defined by the circuit $C$ which gives us an edge-set and the circuit $F$ which colors the vertices of the graph. If there is an invalid edge or a repeated edge, we are done. But if there is not, that means there are $2^{2n-2} + 1$ valid edges in this graph. By Mantel's Theorem, there must exist a triangle amongst these edges. Consider this triangle, and denote its vertices $a$, $b$ and $c$. Since $F$ only colors vertices one of two colors, by the pigeonhole principle, two of these vertices must have the same color. Since these two monochromatic vertices are connected by an edge, we have found a monochromatic edge, and we are done. 

% Note that in the above discussion, our proof of totality did not really make use of the coloring function, $F$. Instead, our proof really relied on the existence of the triangle. It is not surprising, then, that Bad Coloring reduces to Mantel: 

% \begin{theorem}
% 	Bad Coloring Reduces to Mantel
% \end{theorem}

% \begin{proof}
% 	Suppose we are given some instance of the Bad Coloring problem. That is, we are given an edge set function, $C$ and a vertex coloring function, $F$, as in the definition of Bad Coloring. Note that $C$, on its own, defines a Mantel Problem instance. We claim that the certificate from this Mantel Problem instance can serve as a certificate for the Bad Coloring problem. Consider a certificate from the Mantel Problem instance. There are three cases: 
% 	\begin{enumerate}
% 		\item Case 1: The certificate describes an invalid edge. That is, our certificate is an index $i$ such that $C(i)$ produces an edge consisting of two identical vertices. Because both of the problems in question share the same edge-set function, $C$, this index must also be an "invalid edge" certificate for the Bad Coloring Instance. 
% 		\item Case 2: The certificate describes a repeated edge. That is, our certificate contains two distinct indices, $i$ and $j$, where $C(i)$ and $C(j)$ both describe the same set. As in case 1, since both problem instances share the same edge-set function, $C$, this certificate is also a valid certificate for Bad Coloring. 
% 		\item Case 3: The certificate describes a triangle. That is, suppose we have three distinct vertices $i$, $j$, $k$, where $C(i)$, $C(j)$, $C(k)$ describe the edges between the three vertices $a, b, c$. In this case, note that among $F(a), F(b), F(c)$, two of these must be the same. That is, $F$ must assign the same color to at least two of $a, b, c$. Those two vertices are connected. Thus, for those two vertices, the index corresponding to their edge among $i, j, k$, provides a valid monochromatic edge certificate. 
% 	\end{enumerate}
% \end{proof}


% As it turns out, Bad Coloring is PPP-hard. We first begin by introducing some useful basic ideas related to PPP.

% \begin{theorem}
% 	Consider a Pigeonhole Circuit Problem Instance defined by a circuit mapping $n$-bit strings to $n$ -bit strings. This problem is polynomially reducible to a Pigeonhole Circuit Instance defined by a circuit mapping $m$ bitstrings to $m$-bit strings, where $m > n$ and $m = O(poly(n))$. 
% \end{theorem}

% \begin{proof}
% 	Suppose we are given an instance of Pigeonhole Circuit, defined by a circuit $C$:
	
% 	$$C: \{0,1\}^n \mapsto \{0,1\}$$
	
% 	where, as usual, the challenge is to find a $n$-bit string $x$ such that $C(x) = 0$ or two distinct $n$-bit strings, $x$ and $y$, such that $C(x) = C(y)$. We are also given some $m < n$ with $m = O(poly(n))$. Accordingly, we construct a circuit $C'$: 
	
% 	$C' : \{0,1\}^m \mapsto \{0,1\}^m$
	
% 	For the rest of this discussion, we view elements in the domain and range of the above circuits in terms of their decimal representations. For example, $C$ has domain and range in the interval $[0, 2^n-1]$. Viewed in this light, the circuit $C'$ is essentially an extension of the circuit $C$ onto a larger domain (and range). We define $C'$ as follows: consider an input $i$ for $C'$. 
	
% 	\begin{enumerate}
% 		\item If $i$ has a decimal representation which belongs to the domain of $C$, $[0, \dots, 2^{n}-1]$, then, we simply define $C'(i) = C(i)$. 
% 		\item Otherwise, $C(i) = i$ is an identity mapping.
% 	\end{enumerate}
	
% 	Now, for the Pigeonhole Instance problem defined by the circuit $C'$, consider any possible certificate. Suppose the certificate is a zero element; that is, suppose it is an index $i$ such that $C'(i) = 0$. We know that $i$ must be in the domain of $C$, because each index outside of the domain of $C$ is greater than $2^n -1$ and maps to itself. Since $i$ is in the domain of $C$, $C'(i) = C(i) = 0$, and $i$ is a zero element for $C$. Suppose instead that the certificate consists of two distinct indices $i, j$ with $C'(i) = C'(j)$. Once again, both $i$ and $j$ must be in the domain of $C$. To see this, note that if $i$ and $j$ are both outside of the domain of $C$, then $C'(i) = i$ and $C'(j) = j$, and these two values cannot be equal since $i \neq{j}$ by assumption. If instead, $i$ is in the domain of $C$ but $j$ is not, $C'(i) = C(i) \leq{2^n - 1}$, while $C'(j) = j > 2^n  - 1$, so $C'(i) \neq{C'(j)}$. Thus, both $i$ and $j$ are in the domain of $C$, so $C'(i) = C(i) = C'(j) = C(j)$, as desired. 
	
% \end{proof}

% We can argue about the hardness of Bad Coloring (relative to PPP):

% \begin{theorem}
% 	Bad Coloring is PPP-hard. 
% \end{theorem}

% \begin{proof}
% 	Suppose we are given an instance of Pigeonhole Circuit, defined by a circuit $C$:
	
% 	$$C: \{0,1\}^n \mapsto \{0,1\}$$
	
% 	where, as usual, the challenge is to find a $n$-bit string $x$ such that $C(x) = 0$ or two distinct $n$-bit strings, $x$ and $y$, such that $C(x) = C(y)$. We assume that $n$ is an even integer. This is a fair assumption, because if $n$ is an odd integer, we can reduce our Pigeonhole Circuit problem instance to a new Pigeonhole Circuit instance defined on $(n+1)$-bit strings; we have discussed this in a theorem above. 
	
% 	Let $n = 2m$ for some integer $m$. We define a Bad Coloring problem instance on a graph of size $2^{m+1}$. All vertices are encoded by a $(m+1)$-bit string. It remains to define two circuits: 
% 	\begin{enumerate}
% 	    \item $E$ which describes the edge set of the graph 
% 	    \item $F$ which colors the individual vertices of the graph
% 	\end{enumerate}

%      We start by defining the coloring function, $F$: 
	
% 	$$F: \{0,1\}^{m+1} \mapsto \{0,1\} $$
	
% 	The coloring function is defined as follows: for an input $i$, if the leftmost bit of $i$ is $0$, then $F(i) = 0$. Otherwise, $F(i) = 1$. It is clear that there are $2^{m}$ vertices which $F$ maps to $0$ and $2^{m}$ vertices which $F$ maps to $1$. 
	
% 	We now define the circuit $E$, which provides us with an edge set for our graph. 
	
% % 	As a notational convenience, for any two bitstrings $x$ and $y$, $x \circ y$ is the concatenation of $x$ and $y$. 
	
% 	Our edge set contains $2^{2m} + 1 = 2^n + 1$ edges. Accordingly, we define our edge circuit $E$: 
	
% 	$$E: \{0,1\}^{2m+1} \mapsto (\{0,1\}^m) ^2$$
	
% 	and we only consider indices whose decimal representation falls in the interval $[0,2^{2m} ]$. 
	
% 	We now define $E$. For an index $i$ in the interval $[0,2^{2m} ]$, we have:
	
% 	\begin{enumerate}
% 		\item If $i = 2^{2m}$, we let $E(i) = (0^{m+1}, 1\circ 0^m)$. 
% 		\item Otherwise, the index $i$ can be represented by a $2m$-bit string. Let $C(i) = a \circ b$, a concatenation of two $m$-bit strings $a$ and $b$. We define $E(i) = (0 \circ a, 1 \circ b)$. 
% 	\end{enumerate}
	
% 	This completes the definition of the Bad Coloring problem instance. Now it remains to show that any certificate to Bad Coloring gives us a certificate to the original Pigeonhole Circuit problem. There are three types of certificates to Bad Coloring, and we address each type separately. 
	
% 	First, suppose that our certificate provides an invalid edge. That is, we have an index $i$ such that $E(i) = (a,a)$ for some $m+1$-bitstring $m$. Based on the above definition of $E$, this is impossible because every edge contains one string whose leftmost bit is a $0$ and another whose leftmost bit is a $1$. 
	
% 	Second, suppose our certificate describes an edge connecting a monochromatic pair of vertices. That is, our certificate is an index $i$ such that $E(i) = (a,b)$ where $F(a) = F(b)$. This is also impossible based on our definition of $E$. As mentioned above, any edge $i$ contains one bitstring whose leftmost bit is a $0$ and another whose leftmost bit is a $1$. Based on our definition of the coloring function $F$, the former bitstring will be mapped to $0$ and the latter will be mapped to $1$, so these two vertices are not monochromatic.
	
% 	Third, suppose our certificate describes a duplicate edge. That is, our certificate is a pair of distinct indices $i$, $j$ with $E(i)$ and $E(j)$ describing the same edge. This means that $E(i)$ and $E(j)$ contain the same two vertices, which we can express as $0 \circ a$ and $1 \circ b$, where $a$ and $b$ are $m$-bit strings. There are two cases here. First, if either $i$ or $j$ has decimal representation equal to $2^{2m}$, then $E(i) = E(j) = (0^{m+1}, 1 \circ 0^m)$. In this case, one of $i$ or $j$ is \textit{not} equal to $2^{2m}$; suppose without loss of generality that $j\neq{2^{2m}}$. Then by the definition of $E$, $E(j) = (0 \circ 0^{m}, 1 \circ 0^{m})$, which means $C(j) = 0^{2m}$. Thus, $j$ is a zero element of $C$, and we are done. In the second case, suppose neither $i$ or $j$ has a decimal representation equal to $2^{2m}$. Then $E(i) = E(j) = (0 \circ a, 1 \circ b)$, which implies that $C(i) = a\circ b$ and $C(j) = a \circ b$, so $C(i) = C(j)$, providing a collision under $C$. This completes the proof. 
% \end{proof}


% As a result of the above theorem, we have that Mantel is PPP-hard: 

% \begin{theorem}
% 	Mantel is PPP-hard
% \end{theorem}


% Why is Bad Coloring unlikely to be in PPP? The issue is that we do not have any clear way to number the edges of our graph (provided by the circuit $E$). If we had such a numbering/enumeration, we would make a statement about the existence of $2^{2n} + 1$ edges (when there are at most $2^{2n}$ possible edges). We elaborate on this point in the following section.

% \subsection{The Bad Coloring Hierarchy}
% As mentioned above, a graph has no triangles if and only if it is bipartite.
What is the maximum number of edges a bipartite graph can have? This question can be formulated as an optimization problem. Suppose there are $a_0$ nodes on one side of the bipartition and $a_1$ nodes on the other. A bipartition which allows for the largest number of edges will maximize

\begin{equation}
\begin{aligned}
\max \quad {a_0*a_1} \quad\\
\textrm{s.t.}\quad a_0 + a_1 = 2^n & \\ a_0\geq{0}, a_1\geq{0} \\
\end{aligned}
\end{equation}

The solution to the above problem is given by $a = b = 2^{n-1}$, and the maximum number of edges is $2^{2n-2}$. By this logic, no matter how we partition the nodes of the graph, if we are given $2^{2n-2} + 1$ edges, there must be an edge connecting two nodes of the same class. We can (and will) introduce a TFNP problem based on this principle below, which we ``Bad Coloring."  

% Viewed in this light, the Bad Coloring problem gives us an implicit partition of $2^n$ nodes via the coloring function $F$. Further, it gives us a number of edges that is larger than the global optimum of the above optimization problem. We are therefore guaranteed to either have an invalid or repeated edge. 

Can the class PPP be recast in a similar manner? It seems that PPP represents a simpler problem, in which there is no partition; all objects belong to a single class. If there are $2^n$ possible distinct values and we are given a collection of $2^n + 1$ objects, there must be repeated object. 

In the other direction, can we further generalize the argument used above for bipartite graphs? Suppose that we have $k * 2^n$ objects and we partition these nodes into $k$ (as opposed to $2$) distinct classes. Then, suppose we generate all possible ordered $k$-tuples $(a_0, a_1, \dots, a_{k-1})$, where $a_i$ belongs to the $(i+1)$-th class. What is the largest number of distinct $k$-tuples we can generate? 

The answer is given by the global optimum to the following optimization problem: 

\begin{equation}
\begin{aligned}
\max \quad {a_0*a_1*\dots*a_{k-1}} \quad\\
\textrm{s.t.}\quad a_0 + a_1 \dots + a_{k-1}= k * 2^n & \\ \forall{i}, a_i\geq{0} \\
\end{aligned}
\end{equation}

Using a standard method such as Lagrange's Multipliers, it is clear that the global optimum occurs when all $a_i = 2^n$. Therefore, the largest number of distinct $k$-tuples is $2^{kn}$. 

% If we are given $1 + 2^{kn}$ $k$-tuples, one of these $k$-tuples must either have two nodes of the same class or we must have a two identical $k$-tuples. 

Based on this discussion, we can generalize this problem to define a hierarchy of ``Bad Coloring" problems within TFNP. 




\begin{defi}[$k$-Bad Coloring]
    We are given a set $S$ of $k*2^n$ objects which are represented concisely (using $\lceil n + log(k) \rceil$ bits). For clarity, we refer to these objects with the indices $0, 1, 2, \dots, k*2^n - 1$, however all function outputs and inputs represent these objects concisely using $n + log(k)$ bits per object. 
    
    We are given a function, $F$, which assigns each object to one of $k$ distinct classes (or colors): 
    $$F: S \mapsto \{0,1\}^k $$
    
    We are also given a poly(n)-sized circuit, $C$: 
    
    $$C: \{0,1\}^{kn + 1} \mapsto S^k $$
    
    In this problem, we only consider the smallest $2^{kn} + 1$ indices of $C$ and disregard the rest. $C$ takes an index and outputs a tuple of $k$ elements of $S$.
	
	We wish to find one of the following: 
	\begin{enumerate}
% 		\item Invalid tuple: Return an index $i$ in which $C(i)$ contains two identical elements.
		\item Repeated tuple: Return $2$ different indices, $i$ and $j$, which describe the same tuple. This means both $C(i)$ and $C(j)$ contain the exact same elements (though not necessarily in the same order). 
		\item Monochromatic Tuple: Return an index $i$ in which $C(i)$ contains two elements belonging to the same class (as defined by $F$). Note that the two elements can be identical.
	\end{enumerate}
\end{defi}

As suggested above, it is straightforward to see the following: 

\begin{theorem}
    For each positive integer $k$, $k$-Bad Coloring is in TFNP.
\end{theorem}

\begin{theorem}
    PPP is equivalent to $1$-Bad Coloring
\end{theorem} 

% \begin{theorem}
%     Bad Coloring, as defined earlier, is equivalent to $2$-Bad Coloring
% \end{theorem}

Next, we observe that these problems actually form an infinite hierarchy of TFNP search problems. 

\begin{theorem}
    For all nonnegative integers $k$, $k$-Bad Coloring is polynomially reducible to $(k+1)$-Bad Coloring 
\end{theorem}

The proof is fairly straightforward, and we provide it in the appendix. The more interesting question one must ask is why this hierarchy does not collapse onto its base, PPP? The reason for this has to do with the encoding of objects. $1$-Bad Coloring encodes $2^n$ objects using $n$ bits, which is optimal from an information-theoretic standpoint. Subsequent layers of the hierarchy encode $2^{kn}$ objects using $kn + klog(k)$ bits, which is not as efficient. This, in turn, translates to a computationally harder problem at each subsequent level of the hierarchy. 
% \begin{proof}
%     We are given a $k$-Bad Coloring problem instance. In this problem instance, we are given the following:
    
%     \begin{enumerate}
%         \item A set, $S_k$, of $k*2^n$ objects, in which each object is represented by a unique $(n+log(k))$-bit string
%         \item A function $F_k$ which assigns each element of $S_k$ to one of $k$ distinct classes, where each class ($0, 1, \dots, k-1$) is represented in binary: $F_k: S_k \mapsto \{0,1\}^{log(k)}$
%         \item A circuit, $C_k$, which implicitly represents a collection of tuples. Each tuple has size $k$, and $C_k$ provides a total of $2^{kn} + 1$ tuples. Specifically, $C(i)$, for $0\leq{i}\leq{2^{nk} + 1}$ provides a tuple consisting of $k$ elements from $S$.
%     \end{enumerate}
    
%     % we are given a set, $S_k$, of $k*2^n$ objects, in which each object is represented by a unique $(n+log(k))$-bit string. We also are given a function $F_k$ which assigns each element of $S_k$ to one of $k$ distinct classes, where each class ($0, 1, \dots, k-1$) is represented in binary:
    
%     % $$F_k: S_k \mapsto \{0,1\}^{log(k)}$$
    
%     % We are also given a circuit, $C_k$, which implicitly represents a collection of tuples. Each tuple has size $k$, and $C_k$ provides a total of $2^{kn} + 1$ tuples. Specifically, $C(i)$, for $0\leq{i}\leq{2^{nk} + 1}$ provides a tuple consisting of $k$ elements from $S$.
    
%     For clarity of exposition, we refer to all objects and classes in terms of their decimal (as opposed to binary) representations, and note that they are, in reality, concisely represented.
    
%     We now construct a $(k+1)$-Bad Coloring problem instance. This problem has a set, $S_{k+1}$ of size $(k+1)*2^{n}$ objects. We define $S_{k+1} = S_k \bigcup A$, where $A$ is a set of $2^n$ new objects, none of which belong to $S_k$. Thus, $|S_{k+1}| = k*2^n + 2^n = (k + 1)*2^n $. We use the following indexing notation: the smallest $k*2^n$ indices refer to the elements of $S_k$ and the largest $2^n$ indices refer to the elements of $A$. 
    
%     We now define a coloring $F_{k+1}$ over the set $S_{k+1}$. This definition is straightforward: for any $e\in{S_{k+1}$:
%     \begin{enumerate}
%         \item If $e\in{S_k}$, then $F_{k+1}(e) = F_k(e)$
%         \item Otherwise, $F_{k+1}(e) = k$
%     \end{enumerate}
    
%     We now define the circuit $C_{k+1}$, which provides us with a concise representation of $2^{(n*(k+1))} + 1$ tuples, where each tuple contains $k+1$ elements of $S_{k+1}$. We first define $C_{k+1}$ over the smallest $2^{(n)*(k+1)}$ indices.  
%     Let $i$ be such an index. Note that $i$ is represented using $n*(k+1) + 1$ bits. Let $i = a \circ b$ where $a$ is a $1 + n(k)$-bit string and $b$ is a $n$ bit string. Note that $a$ is a valid input for $C_k$. We define $C_{k+1}(i) = C_{k}(a) \bigcup \{x\}$, where $x$ is the $b$-th element of $A$. 
    
%     Now consider $C_{k+1}(i)$ where $i$ has a decimal representation of $2^{(n*(k+1))}$. In this case $i$ can be represented as $i = 1 \circ a \circ b$ where $a$ is a $nk$-bit string consisting of all $0$'s, and $b$ is a $n$-bit string consisting of all $0$'s. We then define $C_{k+1}(i) = C_{k}(1\circ{a}}) \bigcup x$ where $x$ is the  ($0$-th) element of $A$. 
    
%     It remains to show that a certificate for this new problem instance allows us to efficiently recover a certificate to the $k$-Bad Coloring problem instance. Suppose our certificate is an invalid tuple, provided by index $i$.  We know that $C_{k+1}(i)$ takes the form $C_k{x} \bigcup y$ for some $y\in{A}}$ and that the index $x$ can be efficiently calculated from $i$ (from the above definition). Note that $y$ cannot belong to $C_{k}(x)$, and it is not the same color as any element of $C_{k}(x)$ (instead, it is assigned color $k$). Therefore, if $C_{k+1}(i)$ is invalid, there must exist two elements within $C_{k}(x)$ of the same color, making $x$ a valid certificate to the $k$-Bad Coloring problem. 
    
%     Suppose instead that we find a repeated tuple; that is, two distinct indices $i, j$ with $C_{k+1}(i)$ describing the same tuple as $C_{k+1}(j)$. As mentioned above, we know that $C_{k+1}(i) = C_k(x) \bigcap y$, where (from the above definition) it is clear $x$ can be calculated efficiently. By similar reasoning, we can suppose that $C_{k+1}(i) = C_k(a) \bigcap b$. Critically, if $C_{k+1}(i)$ and $C_{k+1}(j)$ are equal, then $y$ must be the same element $b$, and $C_k(x)$ must be identical to $C_k(a)$. Furthermore, $a$ must be distinct from $x$ (if it were not, then $i$ would be identical to $j$). Therefore, $a$ and $x$ form a valid certificate to the original problem. 
% \end{proof}

\fi







==> Konig.tex <==
\section{K\"onig and Erd\H{o}s-Ko-Rado}

In this section we introduce and characterize computational problems associated with two classical theorems in combinatorics.

\subsection{K\"onig}

K\"onig's lemma states that in every infinite connected graph with finite degree there is an infinite path starting at every node.
The lemma is often stated and used for trees: Every infinite (rooted) tree with finite branching has an infinite path (starting at the tree).
The finite version of the lemma is that every large enough graph (or tree) with bounded degree contains a long path. For example, every rooted binary tree with $2^n$ nodes contains a path of length $n$.

The standard proof of K\"onig's lemma (the infinitary as well as the finitary version) is by the same type of repeated majority argument as in the proof of totality for Long Choice. In the general case of an infinite connected graph $G$, 
let $a_0$ be any node. For every other node $u$ fix a canonical path $p(u)$ from $a_0$ to $x$ (it exists because $G$ is connected). Partition the nodes $u$ according to the second node in the path $p(u)$. Since $G$ is infinite and $a_0$ has finite degree, the "largest" group in the partition is infinite, i.e. there is a neighbor $a_1$ of $a_0$ such that $a_1$ is the second node in the path $p(u)$ for an infinite set $S_1$ of nodes $u$. 
Repeat the argument from $a_1$: partition $S_1$ according to the third node in the path $p(u)$; the
"largest" group $S_2$ in the partition is infinite, and all nodes $u \in S_2$ have the same third node $a_2$ in their canonical path $p(u)$.
Continuing in this way will produce an infinite path. 
 

We now introduce computational problems based on Konig's Lemma. We begin by stating the lemma in its most general form.

\begin{theorem}[Konig's Lemma]
	Consider a graph , $G = (V, E)$ with a countably infinite vertex set. Suppose $G$ has the following properties: 
	\begin{enumerate}
		\item The graph is connected
		\item The graph has bounded degree (i.e. each node is connected to at most $m$ nodes for some constant $m$)
	\end{enumerate}

	Konig's Lemma states that from any node, one can construct an infinite simple path.
\end{theorem}

The proof of Konig's Lemma uses essentially the same argument as our of proof of totality for Long Choice.

\begin{proof}
    Consider any node, $a_0$ in the graph $G = (V, E)$. We construct an infinite simple path $a_0, a_1, \dots$ in an inductive fashion. Since $G$ is connected, we know that there exists at least one simple path from $a_0$ to every node of $G$. Let $F$ be a function which takes as input any node from $V$ and outputs a single simple path from $a_0$ to $v$. We call $F(v)$ the ``canonical" path of $v$.
    
    For each of the infinitely many nodes $v\in{V\setminus{\{a_0\}}}$, $F(v)$ has as its second element some neighbor of $a_0$. However, $a_0$ has finitely many neighbors. Therefore, by the infinite pigeonhole principle, there exists a neighbor of $a_0$ which we call $a_1$ with the following property: there are infinitely many vertices which contain a canonical path of the form $a_0, a_1, \dots$.
    
    Consider all vertices $v$ whose canonical path takes the form $a_0, a_1, \dots$. From above, we know there are infinitely many vertices with this property. However, $a_1$ has finitely many neighbors. Therefore, by the Infinite Pigeonhole Principle, there exists a neighbor of $a_1$, which we call $a_2$, with the following property: there are are infinitely many vertices whose canonical path takes the form $a_0, a_1, a_2 \dots $, where $a_2$ is a neighbor of $a_1$. 
    
    We can continue this argument indefinitely to construct an infinite simple path $a_0, a_1, a_2, \dots$. 
\end{proof}

Given a connected graph, how hard is it to find a long simple path? There exists a problem of this form in TFNP, which we call ``Konig" (discussed below). This problem is formulated on a special class of connected, bounded-degree graphs: binary trees. Of course, Konig's Lemma also applies to the special case of binary trees: 

\begin{theorem}[Konig's Lemma: Binary Trees]
	Let $B$ be a binary tree consisting of countably infinitely many nodes. There must exist an infinitely long path starting at the root of $B$.
\end{theorem}

\begin{proof}
    $B$ is a connected graph with bounded degree (in particular, the bound is at most $2$). Therefore, by Konig's Lemma, there exists an infinitely long simple path starting from any node (including the root node). 
\end{proof}

We are now ready to introduce the corresponding search problem in TFNP:

\begin{defi}[Problem: Konig]
	We are given a poly(n)-sized circuit, $P$:
	
	$$P:\mathbb \{0,1\}^{n}\to\mathbb \{0,1 \}^{n} \Cross \{0,1\} $$
	This circuit implicitly defines a tree on $2^n$ nodes, where each node is encoded by a $n$-bit string. It does so by defining a parent relation: for a node $k$, $P(k)$ specifies an ordered pair $(p, s)$ where $p$ is the binary encoding of the parent node of $k$, and $s$ is a bit which specifies whether $k$ is the left or right child of $p$. As a convention, $s = 0$ if $k$ is the left child of $p$, and $s=1$ otherwise. If $P(k) = k$, that means that $k$ does not have a parent (it is a root node). In the Konig problem, we are given a root node, $r$, and asked to find one of the following certificates: 
	
	\begin{enumerate}
		\item \textbf{Identical children: } Return $2$ distinct nodes $a$ and $b$ with the property that $P(a) = P(b)$. (That is, they are both left children or right children of the same node). 
		\item \textbf{Invalid Root: } Return $r$ if $P(r)\neq{r}$.
		\item \textbf{Non-Unique Root: } Return a node $s\neq{r}$ with the property that $P(s) = s$.
		\item \textbf{Far Away Node: } Return a node $s$ with the following property: if we apply the parent operator $P$ to $s$ a total of $n$ times, we do not reach the root $r$. 
		\item \textbf{Long Path: } A sequence of $n+1$ nodes $a_0, a_1, \dots, a_{n}$ with $a_0 = r$, and the property that $P(a_i) = a_{i-1}$ for all $i\geq{1}$. Note that it suffices to provide $a_{n-1}$ as a valid certificate here; the rest of the path can be recovered by applying the parent operator $P$. 
	\end{enumerate}
	
	We refer to the circuit $P$ as the \textbf{parent operator}.
\end{defi}

\begin{figure}[t!]
	\centering
	\includegraphics[width=1\textwidth]{IndexingBinaryTree.png}
	\caption{\textbf{Indexing of a Binary Tree}. Here we provide an illustration of how we index a binary tree in our proof that Konig is PPP-hard. An arrow from node ``a" to node ``b" indicates that ``a" is the parent of ``b". At the top of the image, the root has encoding $0$. Its left child is $1$ and its right child is $2$. Given a node, $x$, the parent function $P$ calculates $P(x) = \lfloor \frac{x-1}{2} \rfloor$.}
	\label{fig:IndexingBinaryTree}
\end{figure}

It turns out that Konig is PPP-complete.

\begin{theorem}
	Konig is PPP-hard
\end{theorem}

\begin{proof}
    We first show that Konig is PPP-hard by providing a reduction from Pigeonhole Circuit. Suppose we are given a circuit $C$ that defines a Pigeonhole Circuit problem instance: 
    
    $$C: \{0,1\}^n \mapsto \{0,1\}^n $$
    
    We define a Konig problem instance, specified by a parent mapping: 
    
    $$P: \{0, 1\}^{n+1} \mapsto \{0,1\}^{n+1} \Cross \{0,1\}$$
    
    Note that $P$ implicitly defines a graph on $2^{n+1}$ vertices. We start by defining the positions of nodes whose binary encodings are in the range $[0, 2^n - 1]$, and we do so recursively. First, $0$ is the root. Next, consider any node $s$ in this range. If the binary encoding of $s$ is odd, we define $P(s) = (\lfloor\frac{s-1}{2} \rfloor, 0)$; that is, $s$ is the left child of a node with binary encoding $\lfloor{\frac{s-1}{2}}\rfloor$. Similarly, if the binary encoding of $s$ is even, we define $P(s) = (\lfloor{\frac{s-1}{2}}\rfloor, 1)$. See Fig.~\ref{fig:IndexingBinaryTree} for an illustration of this structure in the case that $n = 3$. Note that so far, our definition of $P$ has absolutely no dependence on the circuit $C$. 
    
    To finish the above definition of $P$, it remains to consider the nodes whose binary encodings are in the range $A = [2^n, 2^{n+1} - 1]$. Consider a given node $s$ whose encoding lies in the range given by $A$. Then $s - 2^n$ lies in the domain of $C$. Furthermore, for each $s\in{A}$, $s-2^n$ corresponds to a unique element in the domain of $C$. For each $s\in{A}$, we define: 
    
    $$r = C(s - 2^n) + 2^{n} - 1$$
    
    Next, for each $s\in{A}$, we define 
    $$P(s) = (\lfloor \frac{r-1}{2} \rfloor, \text{parity}(C(s-2^n)))$$
    
    where the parity function returns $0$ if the input is even and $1$ if it is odd.
    
    Because the circuit $C$ has range $[0, 2^n-1]$, $r$ must lie in the interval $[2^{n}-1, 2^{n+1}-1]$. Then, based on the definition of $P(s)$, the parent of each $s\in{A}$ must lie in the interval $B = [2^{n-1}-1, 2^{n}-1]$. There are $2^{n-1}$ nodes in the interval $B$, and each of these nodes can have at most $2$ children. Thus, a total of $2^n$ nodes can have parent nodes in the interval $B$.
    
    On the other hand, every node of $A$ must have a parent in the interval $B$, and we know there are $2^n$ nodes in the interval $A$. In addition to the nodes of $A$, we know that the node $2^{n}-1$, which does not belong to $A$, also has a parent in $B$: $P(2^{n}-1) = 2^{n-1}-1$. This implies that a total of $2^n+1$ elements must have a parent belonging to the interval $B$. 
    
    Since $B$ can only have $2^n$ children, by the pigeonhole principle, there must exist a node in $B$ with two left children or two right children. By the definition of the Konig problem, these two left or right children form a valid certificate to the Konig problem. It remains to show that these two nodes also provide a certificate for the Pigeonhole Circuit problem. 
    
    There are two cases to consider. In the first case, suppose that parent node $2^{n-1}-1$ has two left children. We know that one of these children is the node $2^{n}-1$, and the other child must be a node $s\in{A}$. In this case, if $P(s) = (\lfloor \frac{r-1}{2} \rfloor = 2^{n-1}-1, 0)$, we can conclude that $r = 2^{n}-1$. However, this would in turn imply that $C(s - 2^n) = 0$, which means $s - 2^n$ is a zero element to our original Pigeonhole Circuit problem! 
    
    In the second case, suppose that a parent node $i > 2^{n-1}-1$ has two left (or right) children. This would imply that there are two distinct nodes $s_1, s_2\in{A}$ with $P(s_1) = P(s_2)$. By the definition of $P$, this in turn implies that $C(s_1 - 2^n) = C(s_2 - 2^n)$. Since $s_1 \neq{s^2}$, we can conclude that $s_1 - 2^n$ and $s_2 - 2^n$ provide us with a collision in our Pigeonhole Circuit certificate. 
\end{proof}

\begin{theorem}
	Konig is in PPP
\end{theorem}

\begin{proof}
    We are given an instance of the Konig problem, which is defined by a root node, $r$, and a circuit $P$:
    
    $$P: \{0, 1\}^{n} \mapsto \{0,1\}^{n} \Cross \{0,1\}$$
    
    As described above, $P$ implicitly describes a graph on $2^{n}$ nodes. We wish to reduce it to an instance of Pigeonhole Circuit in polynomial time. To do this, we define a circuit, $C$:
    
    $$C: \{0, 1\}^{n} \mapsto \{0,1\}^{n} $$
    
    where the domain of $C$ will be the nodes of the graph defined by $P$.

    In any binary tree, we can assign every node a unique ``index" based on its position relative to the root. This indexing scheme is defined in an inductive fashion. First, the root is given index $0$. Next, suppose a given node $a_i$ has index $i$. Then, we say that its left child has index $2*i + 1$ and its right child has index $2*i + 2$. Fig.~\ref{fig:IndexingBinaryTree} for an illustration of this indexing scheme. 
    
    Consider any node of the graph, $g$. Suppose that $g$ is neither a Far away node nor a Long path certificate nor a Non-unique root. (Note that all of these conditions are easy to verify). Under these assumptions, we show how to can efficiently find the index of $g$. To do this, we repeatedly apply the parent operator, $P$, to the node $g$ until we reach the root node. Based on the assumptions we have made, this is always possible. Furthermore, it will require at most $n-1$ applications of the parent operator. Every time we apply the parent operator to a node, we receive two pieces of information: the node's parent and whether the node is a left or right child of its parent. Thus, once we reach the root node in this process, we have a sequence of nodes $a_0, a_1, a_2, \dots, a_k$ where $a_k = r$ and $a_0 = g$. Furthermore, for each $a_i$ and $a_{i+1}$, we know whether $a_i$ is the left or right child of $a_{i+1}$. We therefore have a path from $r$ to $g$. Using this path, we can use the indexing scheme mentioned above to find the indices of the nodes $r = a_k, a_{k-1}, \dots, a_0 = g$ in that order to finally arrive at the index of node $g$. 
    
    We are now in a position to fully define the circuit $C$. In input $i$, $C(i)$ outputs: 
    
    \begin{enumerate}
        \item $0$ if $r$ is an invalid root
        \item $0$ if $i\neq{r}$ and $i$ is a root (in this case, there is a non-unique root).
        \item $0$ if $i$ is a Far Away Node
        \item $0$ if $i$ provides a certificate for a Long Path.
        \item If \textbf{none} of the above conditions are met, then let $x$ be the index of node $i$ in the binary tree. $C(i)$ returns $x+1$.
    \end{enumerate}
    
    It now remains to show that a certificate to the Konig problem can be recovered from a certificate to the Pigeonhole Circuit problem we have just defined. There are two cases to consider. 
    
    In the first case, suppose our certificate to the Pigeonhole Circuit problem is a zero element. In this case, there are four possibilities. Either $r$ is an invalid root, or $i\neq{r}$ is a root, or $i$ is a Far Away Node or $i$ is a certificate for a Long Path. We can polynomially verify all three of these conditions, and they all represent valid certificates to the Konig problem. 
    
    In the second case, suppose our certificate to the Pigeonhole Circuit problem is a collision of two elements in which neither element is a zero element: $i\neq{j}$ with $C(i) = C(j)\neq{0}$. Then, we know that $i$ and $j$ are not Long Path certificates and are not Far Away nodes. Furthermore, we know that their indices must be equal to each other, which in turn implies that they are left (or right) children of the same parent node. Thus, $i$ and $j$ are identical children and provide us with a valid certificate.
\end{proof}

As a corollary, we can relate Konig to PLC: 

\begin{theorem}
    Konig is in PLC
\end{theorem}

==> LongChoice.tex <==
\section{Long Choice}
We start by recalling the definition of the class PPP.  We first define the problem {\sc Collision} to be the following: we are given a Boolean circuit $C$ with $n$ input bits and $n$ output bits, and we seek either (a) an input $x$ such that $C(x)=0^n$, or (b) a {\em collision}, two distinct inputs $x\neq y$ such that $C(x)=C(y)$.  The class PPP is the set of all search problems that reduce to {\sc Collision.}
For the {\em weak} version of PPP, denoted PWPP, the circuit has $n$ inputs and $n-1$ outputs, and a collision is sought.  It is known that $n-2$ or fewer outputs, down to $n^\delta$ for any $\delta>0$, yield the same class \cite{Komargodski2019}.  

Let us next define the search problem {\sc Ramsey,} motivated by one of the most influential theorems in all of combinatorics: Given a graph with $2^{2n}$ nodes, represented by a circuit with $4n$ input bits
and one output bit, we seek either a clique with $n$ nodes, or an independent set with $n$ nodes. 
The nodes are represented by $2n$-bit strings and the circuit specifies the edge relation of the graph.
%{\sc $r$-color Ramsey} is the generalization where we seek a monochromatic set with $n$ nodes
The well known proof of Ramsey's theorem proceeds by constructing a sequence of $2n$ nodes, where: the first node is arbitrary; and the next node is selected from the available nodes to belong in the {\em majority,} either adjacent or nonadjacent to the last node, whichever group is larger.  In addition, the smaller group becomes unavailable.  Since we start with $2^{2n}$ nodes and the minority becomes unavailable at each step, it is clear that a sequence of $2n$ nodes can be selected, and therein we will find either an independent set or a clique with $n$ nodes.

This proof inspires the key definition of this paper:
\begin{defi} 
The {\sc Long Choice} problem is the following: There is a universe $U$ of $2^n$ objects, represented by the $2^n$ $n$-bit strings.  We are given a sequence of $n-1$ circuits $P_0, \dots, P_{n-2}$, each of poly($n$) size, such that $P_i$ has $(i+2)n$ input bits and one output bit;  circuit $P_i$ represents a {\em predicate} on $i+2$ objects.  We are asked to find a sequence of $n+1$ distinct objects $a_0, \dots, a_{n}$, with the following property: for each $i$ in $[0, \dots, n-2]$, $P_i(a_0, \dots, a_{i},a_{j})$ is the same for all $j>i$.
\end{defi}

\begin{theorem}
{\sc Long Choice} is a total problem in TFNP.
\end{theorem}

\begin{proof}
    Our construction is inspired by the proof of Ramsey's Theorem as well as the two-player game which we described in the introduction. 
    
    First, we pick an arbitrary element $a_0$ in the universe. Then, we partition the remaining elements $a_i$ into two categories, based on the value of $P_0(a_0, a_i)$. Since there are $2^n - 1$ elements being partitioned, the majority of this partition must have at least $2^{n-1}$ elements. We select an arbitrary element $a_1$ from this majority and discard all elements from the minority. 
    
    We then continue this procedure: we partition the remaining elements $x$ based on the value of $P_1(a_0, a_1, x)$, and we pick an arbitrary element $a_2$ from the majority of this new partition. 
    
    We can continue partitioning elements in this fashion and picking elements from the majority until we arrive at a complete Long Choice certificate. This proves the totality of the problem. Membership in TFNP follows from the fact that a candidate certificate sequence $a_0, \ldots a_n$ can be checked easily in polynomial time.
\end{proof}
% \begin{proof}
% Our proof is similar to the method of induced coloring for Ramsey's theorem described in \citep{graham1990ramsey}. 
% Consider a {\sc Long Choice} instance. A valid certificate consists of a sequence of distinct bit strings $x_0, x_1, \dots, x_n$. We show by induction how to construct such a certificate. 
    
%     In our construction, we define a sequence of sets, $S_0 \supset S_1 \supset \dots \supset S_{n-1}$ and a sequence of distinct elements $a_0, \dots, a_n \in{S}$, with the following properties: 
    
%     \begin{enumerate}
%       \item $\forall i\in[0, 1, \dots, n-1]$, we have $|S_i| \geq {2^{n-i}}$
%       \item $\forall i\in[0, 1, \dots, n-1]$, we have $ a_i\in{S_i}$
%       \item $\forall i\in[0, 1, \dots, n-2]$,
%       the value of $P_i(a_0, \ldots, a_i,x)$ is the same $\forall x \in S_{i+1}$
%     \end{enumerate}
    
    
%     As a base case, we begin by defining $S_0 = S$, where $S$ is the universe of all objects in the Long Choice problem instance. Thus, $S_0$ contains $2^n$ elements, and the condition that $|S_i| \geq {2^{n-i}}$ holds for $i = 0$. Next, we arbitrarily pick an element $a_0\in{S_0}$. 
    
%     We now proceed inductively. Suppose that $a_0, \dots, a_{k-1}$ and $S_0 \supset \dots \supset S_{k-1}$ have all been defined in such a way that they satisfy the properties listed above
%     with $k$ in place of $n$.
%     Suppose that $k<n$. We will define $S_k$ and $a_k$ so that the above properties hold also for them.
    
%     Consider the set $T=S_{i-1}\setminus\{a_{i-1}\}$. Partition the set $T$ into two groups,
%     $T_0 = \{ x\in{T}| P_i(a_0, a_1, \dots, a_{i}, x) =0 \}$ and $T_1 = \{ x\in{T} | P_i(a_0, a_1, \dots, a_{i-1}, x) = 1 \}$. Define $S_k$ to be the larger of the two groups $T_0, T_1$ (in case of a tie, pick either one), and define $a_k$ to be an arbitrary element of $S_k$. 
    
%     From the definition of $S_k$ and $a_k$, it is clear that properties 2 and 3 are satisfied.
%     For property 1, we note that $|S_{k-1}| \geq {2^{n-k+1}}$ by the induction hypothesis, hence
%     $|S_k| \geq \lceil \frac{|S_{k-1}-1|}{2} \rceil
%     \geq 2^{n-k}$.
    
%     We can continue this inductive definition to construct a sequence of elements $a_0, \dots, a_{n-1}$ and a sequence of sets $S_{0}, \dots, S_{n-1}$. From the properties of the inductive construction, we know that $|S_{n-1}| \geq 2^{n-(n-1)} = 2$, where one of these elements is $a_{n-1}$. The set $S_{n-1}\setminus \{ {a_{n-1}} \}$ contains at least $1$ element. We define $a_n$ to be any element of $S_{n-1}\setminus \{ {a_{n-1}} \}$ and append it to our sequence to arrive at a final sequence $a_0, a_1, \dots, a_n$.  
    
%     The final sequence, $a_0, \dots, a_n$, has length $n+1$. To show that this sequence forms a valid certificate, consider any predicate function $P_i$, $i\leq n-2$. We have to show that for all $a_j$ with $j > {i}$, $P_i(a_0, \dots, a_i, a_j)$ has the same value. This follows from property 3 and the fact that all $a_j$ with $j>i$ are in $S_{i+1}$, since $a_j \in S_j$ and the sets are nested, hence $S_j \subseteq S_{i+1}$. Therefore, this sequence is a valid certificate to the problem.
% \end{proof}

\if{false}

The above proof provides a seemingly ``inefficient" method to construct a Long Choice certificate. This inefficiency arises for the following reason: at each stage of the above construction we must 

\begin{enumerate}
    \item estimate the majority of a potentially exponentially large set $S_{k-1}$, and 
    \item once we establish this majority (which we define as $S_{k}$), we must find an element from this majority.
\end{enumerate}


It is worth noting that, because of the many choices we make at each stage are somewhat arbitrary. For example, after defining the set $S_k$ in the above proof, we can define $a_k$ to be \textit{any} element in $S_k$ - it does not matter which one. 

The arbitrary nature of choices at each stage of our construction in turn leads to a combinatorial explosion in the number of possible valid certificates. 

\begin{theorem}
    A given Long Choice problem instance with a universe of size $2^n$ objects has at least $2^{n (n+1)/2}$ distinct certificates.
\end{theorem}

\begin{proof}
    Following the proof of totality for Long Choice, recall that when we constructed our certificate, we iteratively defined a sequence of sets $S_0 \supset S_1 \supset \dots \supset S_{n-1}$. At each stage of our construction, once we defined $S_k$, we picked an arbitrary element of $S_k$ and designated this element to be $a_k$. Recall that we showed that $|S_k| > 2^{n-k}$. Thus, to define element $a_k$, there were $2^{n-k}$ choices we could have made. This argument holds for any $k\in [0, 1, \dots, n]$. Therefore, the total number of distinct valid certificates is \textit{at least} 
    $$2^n * 2^{n-1} * \dots * 2^2 * 2^1 * 2^0 = 2^{n * (n+1)/2} $$.
\end{proof}

Does the arbitrary nature of each choice affect the hardness of the problem? We believe this is not the case. Consider an alternative formulation of the Long Choice problem in which the first element of the sequence is constrained to be a certain value, $x$. We call this problem ``Constrained Long Choice". By the above proof of totality, there must exist a valid Long Choice sequence of the form $x, a_1, 
\dots, a_n$. To see why, note that we only need to make one minor modification to the above proof - instead of picking an arbitrary $a_0\in{S}$ as our first element, we pick a \textit{specific} element: $a_0 = x$. 

As it turns out, Long Choice is equivalent to Constrained Long Choice. See the appendix for a detailed proof. 

\begin{theorem}
    Long Choice is equivalent to Constrained Long Choice
\end{theorem}

\textbf{Moving forward, we will be flexible in how we define Long Choice instances. At times, we might explicitly define an initial element, and at times, we might not.} 


\subsection{Relationships between Long Choice and PPP}

\fi 

Critically, {\sc Long Choice} is also PPP-hard. To see why, consider the two-player game from the Introduction which characterizes {\sc Long Choice}. In this game, player 2 can behave (i.e., the predicates $P_i$ can be specified) in a way that guarantees that the only way player 1 wins is by finding a certificate to a PPP-complete problem {\sc Collision.} Consider an instance of {\sc Collision}, given by a circuit, $C$, which maps $n$-bit strings to $n$-bit strings. Player 1 starts the game with $2^n$ objects (the domain of the circuit). At each round, player $1$ picks an element from the remaining set of objects. If at any round, player $1$'s choices so far contain a certificate to {\sc Collision} (that is, one element is a zero element or a pair of elements collide under $C$), then player 2 stops partitioning the remaining elements. That is, player 2, for the rest of the game, places all remaining elements into the same side of the partition, guaranteeing a path to victory for player 1. 

In each round, player $2$ considers the ``vacant spots" in the range of $C$: the nonzero values of the range that do NOT contain the image of player $1$'s choices. 
At round $1$ of the game, player $1$ makes some choice, call it $a_0$. If $C(a_0) = 0$, then player $1$ has found a certificate, and we are done. If $C(a_1)$ is positive, then there are $2^n - 2$ vacant spots left. Player $2$ splits the set of vacant spots into two even halves (there are many ways to do this, one way is for player $2$ to specify a constant, $k$ and declare that all vacant spots less than or equal to $k$ belong to one half, and the vacant spots greater than $k$ belong to the other). 

Regardless of what value player $1$ chooses for $a_1$ in round $2$, all subsequent elements must belong to the same subgroup of $C(a_1)$. After $C(a_1)$ is chosen, the number of vacant spots in this subgroup is $2^{n-1} - 2$. 

% Assuming player $1$ picked from the majority, this means after chosing $a_1$, there are $2^{n-1} - 1$ elements from which player $1$ can still chose. Furthermore, the image of these elements is a set of size $2^{n-1} - 2$ (since we have already picked $a_1$!) By the pigeonhole principle, there must be a collision among these elements. 

The game continues in this fashion, with player $2$ always taking note of the remaining available vacant spots, and splitting this set into $2$ even groups. In general, after the $i$-th round, there will be at most $2^{n-i+1} - 2$ vacant spots left. Therefore, after the $n$-th round, assuming no certificate has yet been found, there will be $2^{1} - 2 = 0$ vacant spots. Therefore, the $(n+1)$-th choice player $1$ makes must provide a collision (or zero element). We provide a complete proof of this result in the appendix.  

\begin{theorem}
{\sc Long Choice} is PPP-hard.
\end{theorem}

% \begin{proof}
% Suppose that we are given a circuit $C_0$ mapping $n$ bits to $n$ bits,  an instance of the {\sc Collision} problem. We can view the inputs and outputs of circuits both as $n$-bit strings or as the equivalent integers in $[0, \ldots, 2^n -1$.  Given $C_0$, we define a new circuit, $C$ which maps $n$-bit strings to $n$-bit strings. On input $a$, we define $C$ as follows:  
	
% 	\begin{enumerate}
% 	    \item $C(a) = 2^n-1$ (the all-1 string) if $C_0(a) = 0$
% 	    \item $C(a) = C_0(a)$ otherwise
% 	\end{enumerate}
	
% 	By the pigeonhole principle, since $C$ only maps inputs to nonzero values, it must have collisions. Any such collision will either allow us to recover a collision in $C_0$ or allow us to recover a zero element of $C$. 
	
% 	We now reduce the problem instance given by circuit $C$ to a Long Choice problem. We begin by defining our set, $S$, to be the domain of circuit $C$: the set of $n$-bit strings. Note that $S$ has $2^n$ distinct elements, each of which is represented as a unique $n$-bit string. It now suffices to define $n-1$ predicate functions $P_0, P_1, \dots, P_{n-2}$.  
	
% 	As in the proof of totality for Long Choice, we can we can think about constructing a certificate by sequentially making the choices $a_0, a_1, \dots, a_n$. Put simply, our predicate functions will classify the elements of $S$ based on their \textit{images} under $C$. These functions will enforce the following property: subsequent elements of our Long Choice certificate will have images under $C$ which are closer and closer together. More specifically, consider the first three elements of a Long Choice certificate, $a_0, a_1, a_2$. While $C(a_0)$ and $C(a_1)$ may be more than $2^{n-1}-1$ units apart, predicate function $P_0$ will enforce the condition that $C(a_1)$ and $C(a_2)$ are within $2^{n-1}-1$ units of each other. Each predicate function will, in effect, enforce similar ``closeness" conditions. Ultimately, this will force any Long Choice certificate to have two distinct elements whose images under $C$ are $0$ units apart (a collision under $C$!), as desired.
	
% 	In the following discussion, we assume all inputs to predicate functions are distinct, because this is required of any valid certificate.
	
% 	We now explicitly define the predicate functions:
% 	\begin{enumerate}
% 		\item $P_i(a_0, \dots, a_i, x) = 1$ if $C(x)$ is in the interval $F_{i}$ (defined below)
% 		\item $P_i(a_0, \dots, a_i, x) = 0$ if $C(x)$ is \textit{not} in the interval $F_{i}$.
% 	\end{enumerate}
	
% 	To complete the definition, we define the intervals, $F_i$, which depend on the elements $a_0, \ldots, a_i$. Before we do so, we introduce some basic terminology to make this discussion clearer.
	
	

% 	\begin{enumerate}
% 		\item \textbf{Unfilled set:} For any sequence of elements $a_0, \dots, a_i$ and an interval $[p, q]$, the unfilled set of the interval is defined as 
		
% 		$$\{ \{p,p+1, \dots, q\}\setminus{\{C(a_0), C(a_1), \dots, C(a_i)\}}\}$$
		
% 		For example, if given a sequence of points $a_0, a_1, a_2$ with $C(a_0) = 0$, $C(a_1) = 2$, $C(a_2) = 1$, the unfilled set for the interval  $[0, 5 ]$ is  $\{3, 4, 5\}$. 
		
%         \item \textbf{Indexing an interval: }(Purely for notational convenience) Given an interval $I = [a,b]$, for $k > 0$, define $I[k]$  as the interval containing the smallest $k$ elements of $I$, and define $I[-k]$ as the interval containing the largest $k$ elements of $I$. For example, given $I = [1,4]$, $I[2] = [1,2 ]$, the first two integers in the interval, while $I[-3] = [2, 4]$, the largest $3$ integers in the interval.
% 	\end{enumerate}
	
	
% 	We now define a sequence of intervals $B_0, \dots, B_i, \dots$ and $F_0, \dots, F_i, \dots$. Critically, each interval $F_i$ is a contained in the corresponding interval $B_i$. We proceed with an inductive definition.
	
	
% 	\textbf{Base Case Definition.}
% 	For any single element sequence $a_0$, the corresponding interval $B_0$ is $[1, 2^n - 1]$. The unfilled set for $B_0$ has size $2^n - 2$. Consider the value of $k$ that guarantees that $B_0[k]$ has an unfilled set of size $2^{n-1}-1$. This can be easily computed:
% 	$k=2^{n-1}-1$ if $C(a_0)> 2^{n-1}-1$, else $k=2^{n-1}$. We define $F_0 = B_0[k]$.
% 	\\[12pt]
% 	\textbf{Inductive Definition.}
% 	Suppose that we have a sequence of elements $a_0, \dots, a_i$, and for all $k<i$, $B_k$ and $F_k$ are defined. We first define $B_i$ using the following rules: 
% 	\begin{enumerate}
% 	    \item First, if $B_{i-1}$ is an interval of size $1$, then $B_i = F_i = B_{i-1}$
% 	    \item Otherwise, if $C(a_i)$ is in $F_{i-1}$, then $B_i = F_{i-1}$. If $C(a_i)$ is not in $F_{i-1}$, then $B_i = B_{i-1}\setminus{F_{i-1}}$.
% 	    \item Finally, we define $F_i$. Let $x$ denote the size of the unfilled set of $B_i$. Let $k$ be the smallest integer such that $B_i[k]$ has $\lceil \frac{x}{2} \rceil$ unfilled spots. We let $F_i = B_i[k]$. 
% 	\end{enumerate}

% 	This completes the definition of the Long Choice problem instance. It remains to prove that a valid certificate for this problem instance allows us to recover a collision under $C$.
% 	Let $a_0, a_1, \ldots, a_n$ be a valid certificate. If there is a collision among these elements, we are done.
% 	So assume there is no collision; we will derive a contradiction.
	
% 	Consider the sequence of set $B_i, F_i$ generated from the sequence $a_0, a_1, \ldots, a_n$.
% 	Note that $B_0\supseteq{B_1}\dots\supseteq{B_i}\dots$ and $F_i \subseteq B_i$ for all $i$.
% 	It is easy to show inductively from the construction that the following two properties hold:\\
% 	1. $\forall i, \forall j \geq i, C(a_j) \in B_i$.\\
% 	2. $|B_i \setminus \{ C(a_0),\ldots, C(a_i)\}| = 2^{n-i}-2$ for all $i \leq n-2$.
	
% 	The basis case ($i=0$) for both properties is trivial. The induction step for property 1 follows from the fact that $P_{i-1}(a_0,\ldots,a_{i-1},a_j)$ has the same value for all $j \geq i$, hence either all these $a_j$ are in $F_{i-1}$ or they are all not in $F_{i-1}$ and thus they are in $B_{i-1} \setminus F_{i-1}$ (because they are all in $B_{i-1}$ by the induction hypothesis). It follows from the definition of $B_i$ that they are all in $B_i$.
	
% 	For the induction step of property 2 note that the induction hypothesis $|B_{i-1} \setminus \{ C(a_0),\ldots, C(a_{i-1})\}| = 2^{n-i+1}-2$ implies that both $F_{i-1}$ and $B_{i-1} \setminus F_{i-1}$ have $2^{n-i}-1$ unfilled spots. Since $a_i \in B_i$ and $a_i$ does not collide with any earlier $a_j$, it follows that $|B_i \setminus \{ C(a_0),\ldots, C(a_i)\}| = 2^{n-i}-2$.
	
% 	From property 2, $B_{n-2}$ has an unfilled set of size $2^2 - 2 = 2$. The interval $F_{n-1}$ is, by definition, constructed such that $F_{n-1}$ and $B_{n-2}\setminus{F_{n-1}}$ both have $1$ unfilled spot. Critically, based on the definition of $P_{n-2}$, we know that $C(a_{n-1})$ and $C(a_{n})$ must both belong to $F_{n-1}$ or both belong to $B_{n-2}\setminus{F_{n-1}}$. Therefore,
% 	$C(a_{n-1})$ and/or $C(a_{n})$ must collide with each other or with another element in the sequence, a contradiction. 
% \end{proof}

\if{false}

As discussed above, {\sc Long Choice} is a total problem, and this totality is guaranteed by an iterated pigeonhole principle argument. In particular, we have shown that given a universe of \textit{at least} $2^n$ distinct objects, there exists a Long Choice sequence of length $n + 1$. Is this extremal bound of $2^n$ elements optimal? Based on the above reduction from PPP, we can argue that it is indeed optimal. 

\begin{theorem}
    The Long Choice problem must have a universe of at least $2^n$ elements to guarantee the existence of a Long Choice sequence consisting of $n+1$ elements. 
\end{theorem}

\begin{proof}
    We know from the proof of totality for Long Choice (given above) that if the problem has a universe consisting of at least $2^n$ objects, it necessarily has a Long Choice certificate. 
    
    What is left to show is that $2^n$ is the smallest possible size of the universe over which a solution is guaranteed to exist. To do this, we construct an instance of a Long Choice problem which has a universe of $2^n - 1$ elements and argue that it has no valid Long Choice certificate. 
    
    Consider the following mapping: 
    
    To do this, consider a mapping $C$: 
    
    $$C: \{0, 1, \dots, 2^n - 2 \} \mapsto \{0, 1, 2, \dots, 2^n - 1\} $$
    
    where $C(i) = i + 1$. This mapping can be concisely represented by a circuit (a simple circuit which adds $1$ to its input). Note that this circuit maps $2^n - 1$ elements from the domain into $2^n - 1$ distinct elements in the range. Furthermore, it has no zero elements or colliding elements (which we would expect from a normal circuit in the Pigeonhole Circuit problem). 
    
    Now, we define a Long Choice problem instance. To do so, recall the reduction (given above) from the Pigeonhole Circuit problem to Long Choice. In this reduction, we started with a circuit, $E$, mapping elements into the range $\{0, 1, \dots, 2^n - 1 \}$ and we finished with a Long Choice problem instance whose universe consisted of the \textit{domain} of $E$. The resulting problem instance had the property that any valid Long Choice certificate can be used to recover a collision or zero elements of $E$. 
    
    In this proof, we follow the exact same reduction starting from the circuit $C$. The end result of this reduction is a Long Choice problem instance with a universe of $2^n - 1$ (as opposed to $2^n$) elements. This problem instance has the property that any Long Choice certificate will allow us to efficiently recover a collision or zero element in the circuit $C$. However, by the above construction, we know $C$ does not have any zero elements or collisions. Therefore, there are no valid Long Choice certificates in this problem instance. 
\end{proof}

If we think of Long Choice certificates as combinatorial structures, the above proof gives us an explicit construction of a universe (and associated predicate functions) in which there are no Long Choice sequences. In contrast, the problem of explicitly constructing large graphs with no clique or disjoint set (so-called Ramsey graphs) has been a challenging problem. 


% \subsection{PWPP and Long Choice}
% In this section, we explain a useful relation between a weaker version of Long Choice and PWPP. 
\fi
% We next consider the following version of Long Choice in which all predicate functions are binary predicates. 

Several problems reduce to simplified cases of Long Choice where the predicates have fixed arity.
Define {\sc Unary Long Choice} to be the version of Long Choice where every predicate $P_i$ depends only on its last argument,
i.e., $P_i(a_0,\ldots, a_i,x) = P_i(x)$.
Define {\sc Binary Long Choice} to be the version of Long Choice where every predicate $P_i$ depends only on two of its arguments, the last argument $x$ and one of the previous $a_k$, i.e. $P_i(a_0,\ldots, a_i,x) = P_i(a_k,x)$ for some $k \leq i$.


It is easy to see that PWPP reduces to {\sc Unary Long Choice}:
Given a circuit $C$ for PWPP with $n$ input bits and $n-1$ output bits, define $P_i(x)$ to be the $(i+1)$-th bit of $C(x)$. Then in any valid certificate $a_0, \ldots, a_{n-1}, a_n$ for this instance of {\sc Unary Long Choice}, we must have $C(a_{n-1}) = C(a_n)$. 

\if{false}
We can consider a simplified version of Long Choice, in which each predicate function has an arity of $2$: 

\begin{defi}[Problem: Binary Long Choice]
	Consider a set $S$ of $2^n$ objects, $\{a_i\}$, each represented by a unique $n$-bit string. We are given a sequence of $n-1$ predicate functions, $P_0, \dots, P_{n-2}$. Each of these predicate functions are represented as poly(n)-sized circuits. Predicate function $P_i$ has arity $2$: 
	$$ P_i : S^{2} \mapsto \{0,1\}$$
	The problem is to find:
	\begin{enumerate}
		\item \textbf{Long Choice: }A sequence of $n+1$ distinct points $a_0, \dots, a_{n}\in{S}$, with the property that for every $i$ in $[0, \dots, n-2]$, $P_i(a_{i},a_{j})$ is the same for all $j > i$.
	\end{enumerate}
\end{defi}

% This problem is a specialization of the original Long Choice problem, in which the arity of each predicate function is $2$. Therefore, it is a total problem.
As it turns out, this simplified problem captures the complexity of the class PWPP; see the appendix for a complete proof. 
\fi

\begin{theorem}
	PWPP reduces to {\sc Unary Long Choice}.
\end{theorem}

In the next section we will see that Ramsey problems reduce to {\sc Binary Long Choice}.

% \begin{proof}
% 	We are given an instance of PWPP(n, n-1), defined by a circuit $C$: 
	
% 	$$C: \{0,1\}^n \mapsto \{0,1\}^{n-1} $$
	
% 	We wish to find a collision. 
	
% 	We build a Binary Long Choice problem instance with a universe of objects belonging in the set $\{0,1\}^n$. We can now define our predicate functions. For function $P_i$, on distinct inputs $a_i, a_k$, $P_i(a_i, a_k)$ outputs the $(i+1)$-th bit of $C(a_k)$.


% 	Each predicate function $P_i$ enforces a condition on the elements $a_j$, where $j > i$. In particular, $P_i$ requires that for every $j, k > i$, the $(i+1)$-th bits of $C(a_j)$ and $C(a_k)$ agree. Now, consider the last two elements of our Long Choice sequence: $a_{n-1}$ and $a_n$. Following the above reasoning, the predicate functions $P_0, \dots, P_{n-2}$ enforce that $C(a_{n-1})$ and $C(a_n)$ agree over all of their $n-1$ bits, implying that they collide. Thus, a certificate for our Long Choice problem provides us with a valid certificate for the original PWPP-complete problem.
% \end{proof}

% \subsection{Long Choice with Order}
In the opposite direction, we can make the Long Choice problem harder by requiring the elements $a_i$ in the certificate to satisfy additional conditions, while still preserving the totality of the problem; for example we can require the $a_i$ to satisfy a given total order. In the proof of the totality of {\sc Long Choice}, we partition in each step the currently available set and pick an arbitrary element from the majority. We can instead pick a specific element, e.g. the smallest element under the given ordering. We call this generalization {\sc Long Choice with Order}; see the appendix for a formal definition. 

% \begin{defi}[Long Choice with Order]
% 	Consider a set $S$ of $2^n$ objects, $\{a_i\}$, each represented by a unique $n$-bit string. We are given a sequence of $n-1$ predicate functions, $P_0, \dots, P_{n-2}$. Predicate function $P_i$ has arity $i + 2$: 
% 	$$ P_i : S^{i+1} \mapsto \{0,1\}$$
% 	The $P_i$ are concisely represented. We are also given a function $F$ which defines a strict total order over the above set $S$. The function $F$ is also concisely represented by a circuit: 
	
% 	$$F: S^2 \mapsto \{0,1\} $$
% 	Given two distinct inputs $a_x, a_y$, $F(a_x, a_y) = 0$ indicates that $a_x < a_y$ in this total ordering. $F(a_x, a_y) = 1$ indices that $a_x > a_y$. The problem is to find any of the following:
% 	\begin{enumerate}
% 		\item \textbf{Long Choice: }A monotone increasing sequence of $n+1$ distinct points in $S$, $a_0, \dots, a_{n}$, with the following property: for each $i$ in $[0, \dots, n-2]$, $P_i(a_0, \dots, a_{i},a_{j})$ is the same whenever $j > i$.
% 		\item \textbf{Order Violation: } A set of $3$ distinct objects $a_x, a_y, a_z$ which violate the transitivity property of total orders.
% 	\end{enumerate}
% \end{defi}

% This problem is total for essentially the same reason Long Choice is a total problem, but this time, we pick the smallest element available at each stage to ensure we satisfy the ordering requirement.  

% We can apply the exact same argument we did to prove Long Choice is total; the only difference is that instead of making arbitrary choices $a_i$ at each step, we now deliberately pick the \textit{smallest} available choice. Assuming the total order $F$ is valid, this is always possible. 


==> PPPcompleteExtremal.tex <==
\section{K\"onig and Erd\H{o}s-Ko-Rado}

In this section we introduce and characterize computational problems associated with two classical theorems in combinatorics.

\subsection{K\"onig}

K\"onig's lemma states that in every infinite connected graph with finite degree there is an infinite simple path starting at every node.
The lemma is often stated and used for trees: Every infinite (rooted) tree with finite branching has an infinite path (starting at the root).
The finite version of the lemma is that every large enough connected graph (or tree) with bounded degree contains a long path. For example, every rooted binary tree with $2^n$ nodes contains a path of length $n$.
The graph version follows easily from the tree version: Given a connected graph, take a spanning tree of the graph, for example a breadth-first-tree from an arbitrary node.

The standard proof of K\"onig's tree lemma (both the infinitary as well as the finitary version) is by the same type of repeated majority argument as in the proof of totality for Long Choice. 
Starting from the root of the tree, proceed to the
child whose subtree contains the largest number of nodes, and repeat the process from there.
If the tree is infinite, one of the children must have an infinite subtree (since the degree is finite), thus this process will generate an infinite path. Similarly, in the finite case, every iteration reduces the number of nodes at most by a factor of $d$ (the degree), so the process generates a path of logarithmic length.


\if{false}

\begin{theorem}[Konig's Lemma]
	Consider a graph , $G = (V, E)$ with a countably infinite vertex set. Suppose $G$ has the following properties: 
	\begin{enumerate}
		\item The graph is connected
		\item The graph has bounded degree (i.e. each node is connected to at most $m$ nodes for some constant $m$)
	\end{enumerate}

	Konig's Lemma states that from any node, one can construct an infinite simple path.
\end{theorem}

The proof of Konig's Lemma uses essentially the same argument as our of proof of totality for Long Choice.

\begin{proof}
    Consider any node, $a_0$ in the graph $G = (V, E)$. We construct an infinite simple path $a_0, a_1, \dots$ in an inductive fashion. Since $G$ is connected, we know that there exists at least one simple path from $a_0$ to every node of $G$. Let $F$ be a function which takes as input any node from $V$ and outputs a single simple path from $a_0$ to $v$. We call $F(v)$ the ``canonical" path of $v$.
    
    For each of the infinitely many nodes $v\in{V\setminus{\{a_0\}}}$, $F(v)$ has as its second element some neighbor of $a_0$. However, $a_0$ has finitely many neighbors. Therefore, by the infinite pigeonhole principle, there exists a neighbor of $a_0$ which we call $a_1$ with the following property: there are infinitely many vertices which contain a canonical path of the form $a_0, a_1, \dots$.
    
    Consider all vertices $v$ whose canonical path takes the form $a_0, a_1, \dots$. From above, we know there are infinitely many vertices with this property. However, $a_1$ has finitely many neighbors. Therefore, by the Infinite Pigeonhole Principle, there exists a neighbor of $a_1$, which we call $a_2$, with the following property: there are are infinitely many vertices whose canonical path takes the form $a_0, a_1, a_2 \dots $, where $a_2$ is a neighbor of $a_1$. 
    
    We can continue this argument indefinitely to construct an infinite simple path $a_0, a_1, a_2, \dots$. 
\end{proof}

\fi

Given a (succinctly represented) exponentially large connected graph or tree with bounded degree, e.g. a binary tree, how hard is it to find a long simple path? We formulate this problem below for binary trees, represented through the parent information.  

% Of course, Konig's Lemma also applies to the special case of binary trees: 

% \begin{theorem}[Konig's Lemma: Binary Trees]
% 	Let $B$ be a binary tree consisting of countably infinitely many nodes. There must exist an infinitely long path starting at the root of $B$.
% \end{theorem}

% \begin{proof}
%     $B$ is a connected graph with bounded degree (in particular, the bound is at most $2$). Therefore, by Konig's Lemma, there exists an infinitely long simple path starting from any node (including the root node). 
% \end{proof}

% We are now ready to introduce the corresponding search problem in TFNP:

\begin{defi}[Problem: \sc{K\"onig}]
	We are given a poly(n)-sized circuit, $P:\mathbb \{0,1\}^{n}\to\mathbb \{0,1 \}^{n} \Cross \{0,1\} $.
	This circuit is supposed to define a rooted binary tree on $2^n$ nodes, where each node is encoded by a $n$-bit string. It does so by defining a parent relation: for a node $u$, $P(u)$ is an ordered pair $(v, b)$ where $v$ is the (binary encoding of) the parent of $u$, and $b$ is a bit which indicates whether $u$ is the left or right child of $v$. 
	%As a convention, $s = 0$ if $k$ is the left child of $p$, and $s=1$ otherwise. 
	If $P(u) = u$, that means that $u$ does not have a parent (it is a root node). In the K\"onig problem, we are given $P$ and a root node, $r$, and are asked to find either a violation ($P$ does not specify a binary tree rooted at $r$) or find a path of length $n$. Specifically, return one of the following certificates: 
	
	\begin{enumerate}
		\item \textbf{Identical children: } Return $2$ distinct nodes $a$ and $b$ with the property that $P(a) = P(b)$. (That is, they are both left children or right children of the same node). 
		\item \textbf{Invalid Root: } Return $r$ if $P(r)\neq{r}$.
		\item \textbf{Non-Unique Root: } Return a node $s\neq{r}$ with the property that $P(s) = s$.
		\item \textbf{Far Away Node: } Return a node $s$ with the following property: if we apply the parent operator $P$ to $s$ a total of $n$ times, we do not reach the root $r$. 
		\item \textbf{Long Path: } A sequence of $n+1$ nodes $a_0, a_1, \dots, a_{n}$ with $a_0 = r$, and the property that $P(a_i) = a_{i-1}$ for all $i\geq{1}$. Note that it suffices to provide $a_{n-1}$ as a valid certificate here; the rest of the path can be recovered by applying the parent operator $P$. 
	\end{enumerate}
\end{defi}	
We refer to the circuit $P$ as the {\em parent operator}. 
In cases 1, 2, 3, $P$  does not induce a binary tree. The same is true in case 4, if applying $P$ to $s$ $n$ times produces a repeated node; otherwise, we get a simple path of length $n$. Case 5 yields a path of length $n$ from the root $r$.


% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=1\textwidth]{IndexingBinaryTree.png}
% 	\caption{\textbf{Indexing of a Binary Tree}. Here we provide an illustration of how we index a binary tree in our proof that Konig is PPP-hard. An arrow from node ``a" to node ``b" indicates that ``a" is the parent of ``b". At the top of the image, the root has encoding $0$. Its left child is $1$ and its right child is $2$. Given a node, $x$, the parent function $P$ calculates $P(x) = \lfloor \frac{x-1}{2} \rfloor$.}
% 	\label{fig:IndexingBinaryTree}
% \end{figure}

The proof of K\"onig's lemma suggests that the problem should be in PLC. It turns out that {\sc K\"onig}
is in fact in PPP, and furthermore it is complete; see the appendix for a formal proof.

\begin{theorem}
    {\sc K\"onig} is PPP-complete.
\end{theorem}

% \begin{theorem}
% 	Konig is PPP-hard
% \end{theorem}

% \begin{proof}
%     We first show that Konig is PPP-hard by providing a reduction from Pigeonhole Circuit. Suppose we are given a circuit $C$ that defines a Pigeonhole Circuit problem instance: 
    
%     $$C: \{0,1\}^n \mapsto \{0,1\}^n $$
    
%     We define a Konig problem instance, specified by a parent mapping: 
    
%     $$P: \{0, 1\}^{n+1} \mapsto \{0,1\}^{n+1} \Cross \{0,1\}$$
    
%     Note that $P$ implicitly defines a graph on $2^{n+1}$ vertices. We start by defining the positions of nodes whose binary encodings are in the range $[0, 2^n - 1]$, and we do so recursively. First, $0$ is the root. Next, consider any node $s$ in this range. If the binary encoding of $s$ is odd, we define $P(s) = (\lfloor\frac{s-1}{2} \rfloor, 0)$; that is, $s$ is the left child of a node with binary encoding $\lfloor{\frac{s-1}{2}}\rfloor$. Similarly, if the binary encoding of $s$ is even, we define $P(s) = (\lfloor{\frac{s-1}{2}}\rfloor, 1)$. See Fig.~\ref{fig:IndexingBinaryTree} for an illustration of this structure in the case that $n = 3$. Note that so far, our definition of $P$ has absolutely no dependence on the circuit $C$. 
    
%     To finish the above definition of $P$, it remains to consider the nodes whose binary encodings are in the range $A = [2^n, 2^{n+1} - 1]$. Consider a given node $s$ whose encoding lies in the range given by $A$. Then $s - 2^n$ lies in the domain of $C$. Furthermore, for each $s\in{A}$, $s-2^n$ corresponds to a unique element in the domain of $C$. For each $s\in{A}$, we define: 
    
%     $$r = C(s - 2^n) + 2^{n} - 1$$
    
%     Next, for each $s\in{A}$, we define 
%     $$P(s) = (\lfloor \frac{r-1}{2} \rfloor, \text{parity}(C(s-2^n)))$$
    
%     where the parity function returns $0$ if the input is even and $1$ if it is odd.
    
%     Because the circuit $C$ has range $[0, 2^n-1]$, $r$ must lie in the interval $[2^{n}-1, 2^{n+1}-1]$. Then, based on the definition of $P(s)$, the parent of each $s\in{A}$ must lie in the interval $B = [2^{n-1}-1, 2^{n}-1]$. There are $2^{n-1}$ nodes in the interval $B$, and each of these nodes can have at most $2$ children. Thus, a total of $2^n$ nodes can have parent nodes in the interval $B$.
    
%     On the other hand, every node of $A$ must have a parent in the interval $B$, and we know there are $2^n$ nodes in the interval $A$. In addition to the nodes of $A$, we know that the node $2^{n}-1$, which does not belong to $A$, also has a parent in $B$: $P(2^{n}-1) = 2^{n-1}-1$. This implies that a total of $2^n+1$ elements must have a parent belonging to the interval $B$. 
    
%     Since $B$ can only have $2^n$ children, by the pigeonhole principle, there must exist a node in $B$ with two left children or two right children. By the definition of the Konig problem, these two left or right children form a valid certificate to the Konig problem. It remains to show that these two nodes also provide a certificate for the Pigeonhole Circuit problem. 
    
%     There are two cases to consider. In the first case, suppose that parent node $2^{n-1}-1$ has two left children. We know that one of these children is the node $2^{n}-1$, and the other child must be a node $s\in{A}$. In this case, if $P(s) = (\lfloor \frac{r-1}{2} \rfloor = 2^{n-1}-1, 0)$, we can conclude that $r = 2^{n}-1$. However, this would in turn imply that $C(s - 2^n) = 0$, which means $s - 2^n$ is a zero element to our original Pigeonhole Circuit problem! 
    
%     In the second case, suppose that a parent node $i > 2^{n-1}-1$ has two left (or right) children. This would imply that there are two distinct nodes $s_1, s_2\in{A}$ with $P(s_1) = P(s_2)$. By the definition of $P$, this in turn implies that $C(s_1 - 2^n) = C(s_2 - 2^n)$. Since $s_1 \neq{s^2}$, we can conclude that $s_1 - 2^n$ and $s_2 - 2^n$ provide us with a collision in our Pigeonhole Circuit certificate. 
% \end{proof}

% \begin{theorem}
% 	Konig is in PPP
% \end{theorem}

% \begin{proof}
%     We are given an instance of the Konig problem, which is defined by a root node, $r$, and a circuit $P$:
    
%     $$P: \{0, 1\}^{n} \mapsto \{0,1\}^{n} \Cross \{0,1\}$$
    
%     As described above, $P$ implicitly describes a graph on $2^{n}$ nodes. We wish to reduce it to an instance of Pigeonhole Circuit in polynomial time. To do this, we define a circuit, $C$:
    
%     $$C: \{0, 1\}^{n} \mapsto \{0,1\}^{n} $$
    
%     where the domain of $C$ will be the nodes of the graph defined by $P$.

%     In any binary tree, we can assign every node a unique ``index" based on its position relative to the root. This indexing scheme is defined in an inductive fashion. First, the root is given index $0$. Next, suppose a given node $a_i$ has index $i$. Then, we say that its left child has index $2*i + 1$ and its right child has index $2*i + 2$. Fig.~\ref{fig:IndexingBinaryTree} for an illustration of this indexing scheme. 
    
%     Consider any node of the graph, $g$. Suppose that $g$ is neither a Far away node nor a Long path certificate nor a Non-unique root. (Note that all of these conditions are easy to verify). Under these assumptions, we show how to can efficiently find the index of $g$. To do this, we repeatedly apply the parent operator, $P$, to the node $g$ until we reach the root node. Based on the assumptions we have made, this is always possible. Furthermore, it will require at most $n-1$ applications of the parent operator. Every time we apply the parent operator to a node, we receive two pieces of information: the node's parent and whether the node is a left or right child of its parent. Thus, once we reach the root node in this process, we have a sequence of nodes $a_0, a_1, a_2, \dots, a_k$ where $a_k = r$ and $a_0 = g$. Furthermore, for each $a_i$ and $a_{i+1}$, we know whether $a_i$ is the left or right child of $a_{i+1}$. We therefore have a path from $r$ to $g$. Using this path, we can use the indexing scheme mentioned above to find the indices of the nodes $r = a_k, a_{k-1}, \dots, a_0 = g$ in that order to finally arrive at the index of node $g$. 
    
%     We are now in a position to fully define the circuit $C$. In input $i$, $C(i)$ outputs: 
    
%     \begin{enumerate}
%         \item $0$ if $r$ is an invalid root
%         \item $0$ if $i\neq{r}$ and $i$ is a root (in this case, there is a non-unique root).
%         \item $0$ if $i$ is a Far Away Node
%         \item $0$ if $i$ provides a certificate for a Long Path.
%         \item If \textbf{none} of the above conditions are met, then let $x$ be the index of node $i$ in the binary tree. $C(i)$ returns $x+1$.
%     \end{enumerate}
    
%     It now remains to show that a certificate to the Konig problem can be recovered from a certificate to the Pigeonhole Circuit problem we have just defined. There are two cases to consider. 
    
%     In the first case, suppose our certificate to the Pigeonhole Circuit problem is a zero element. In this case, there are four possibilities. Either $r$ is an invalid root, or $i\neq{r}$ is a root, or $i$ is a Far Away Node or $i$ is a certificate for a Long Path. We can polynomially verify all three of these conditions, and they all represent valid certificates to the Konig problem. 
    
%     In the second case, suppose our certificate to the Pigeonhole Circuit problem is a collision of two elements in which neither element is a zero element: $i\neq{j}$ with $C(i) = C(j)\neq{0}$. Then, we know that $i$ and $j$ are not Long Path certificates and are not Far Away nodes. Furthermore, we know that their indices must be equal to each other, which in turn implies that they are left (or right) children of the same parent node. Thus, $i$ and $j$ are identical children and provide us with a valid certificate.
% \end{proof}

%As a corollary, we can relate Konig to PLC: 

%\begin{theorem}
%    Konig is in PLC
%\end{theorem}

\subsection{Erd\H{o}s-Ko-Rado}

The Erd\H{o}s-Ko-Rado Lemma is one of the foundational results in extremal set theory.

% These definitions/ideas are taken from the textbook, ``Extremal Problems for Finite Sets", by Frankl. 


% \begin{defi}[$k$-Subsets]
% 	Consider a finite set $X$, and fix positive integer $k$ with $k < |X|$. We define $X\choose{k}$ to be the set of subsets of $X$ that have size $k$. That is,  $X\choose{k} $ $= \{U | U\subset{X}, |U| = k\}$.
% \end{defi}


% \begin{defi}[Intersecting Set System]
% 	An intersecting set system, $F$, is a collection of finite sets whose pairwise intersections are nonempty. In other words, $\forall a, b \in{F}, a\cap{b} \neq{\emptyset}$.
% \end{defi}

\begin{theorem}[Erd\H{o}s-Ko-Rado Lemma]
If $F$ is any $k$-set system over a universe $X$ of size $n > 2k$, and every pair of sets in $F$ has non-empty intersection, then
	$$|F| \leq {{n-1}\choose{k-1}} $$.
\end{theorem}


Thus, if $|F| > {{n-1}\choose{k-1}} $ then $F$ must contain two disjoint sets. How hard is it to \textit{find} these two disjoint sets, if $F$ is a succinctly given exponentially large system? 

Take the case in which $k = 2$ and the size of the universe is $2^n$. In this case, the Erdos-Ko-Rado lemma tell us that the largest possible intersecting set system has size ${{2^n - 1}\choose{1}} = 2^n-1$. Therefore, given a $2$-set system $F$ of size $2^n > 2^n - 1$, then $F$ must contain two disjoint sets. 

\begin{defi}[Problem Statement: {\sc Erd\H{o}s-Ko-Rado}]
   We are given a poly($n$)-sized circuit
   $$F: \{0,1\}^n \mapsto (\{0,1\}^n)^2 $$
   which is supposed to represent a 2-set system of size $2^n$ over the universe $X=\{0,1\}^n$.
   The problem is to find either a violation ($F$ is not a valid encoding) or two disjoint sets of the set system. Specifically, return one of the following certificates: 
	\begin{enumerate}
    \item (Error:)	An index $i$ such that $F(i)=(a,a)$ for some $a \in \{0,1\}^n$ (i.e., the set $F(i)$ has two identical elements), or two distinct indices $i ,j$ such that the sets (represented by) $F(i), F(j)$ are equal, or
    \item (Disjoint sets:) Two indices $i, j$ such that the sets (represented by) $F(i), F(j)$ are disjoint.
%		\item Invalid set: Find an input, $i$ such that $F(i) = (a,a)$. A set cannot have two identical elements, hence the name "invalid set."
%		\item Repeated set: Find distinct inputs, $i$ and $j$ such that $F(i)$ and $F(j)$ output the same set. That is, each of $F(i)$ and $F(j)$ outputs either $(a,b)$ or $(b,a)$ for some $a, b\in{X}$. 
%		\item Disjoint set: Find inputs, $i$ and $j$, such that $F(i)$ and $F(j)$ are disjoint. 
	\end{enumerate} 
\end{defi}

By the Erd\H{o}s-Ko-Rado lemma, one of these conditions must occur, placing the problem in TFNP. 

In the Appendix we show the following: 
% For any such problem, a witness is guaranteed to exist. Consider any instance of the Erdos-Ko-Rado problem. In this situation, if there is an invalid set, we are done. If there is a repeated set, we are done. If there are no invalid or repeated sets, then we have a $2$-set system over the universe $[0,2^n - 1]$ with $2^n$ elements. By the Erdos-Ko-Rado Lemma, there must be a disjoint set. Therefore, this problem is in TFNP. 


\begin{theorem}
	{\sc Erd\H{o}s-Ko-Rado} is PPP-complete. 
\end{theorem}

 

% \begin{proof}
% 	We first prove that Erdos-Ko-Rado is PPP-hard. Accordingly, suppose we are given some instance of Pigeonhole Circuit, a PPP-complete problem. This problem is defined by a circuit, $C$: 
% 	$$C: \{0,1\}^n \mapsto \{0,1\}^n $$
% 	and the challenge is to find an input that maps to $0$ or find two distinct inputs which map to the same value. 
	
% 	We construct a circuit, $F$, which implicitly defines a $2$-set system of size $2^n$. Our circuit $F$ takes, as input, an $n$-bit string, and outputs a $(\{0,1\}^n)^2$-bit string: $F(x) = (0^n, C(x))$.
	
% % 	\begin{enumerate}
% % 		\item Case 1: $C(x) \neq{0^n}$. In this case, $F(x) = (0^n, C(x))$. 
% % 		\item Case 2: $C(x) = 0$. In this case, $F(x) = (0^n, 0^n)$. 
% % 	\end{enumerate}
	
% 	It remains to show that any solution to this instance of the Erdos-Ko-Rado problem allows us to recover a solution to the original Pigeonhole Circuit problem. There are $3$ possible types of certificates that we can find in the Erdos-Ko-Rado problem instance. FIrst, consider a certificate providing a disjoint set. This is impossible from the above definition of $F$, since every set contains the element $0$. Second, consider a certificate providing an invalid set. This can only happen in Case 2 listed above. In that case, we find a zero element in the Pigeonhole Circuit problem. Third, consider a certificate which defines a repeat set. That is, we have two indices $a$ and $b$ with $F(a)$ and $F(b)$ defining the same set. As we see in the above definition of $F$, this implies that $C(a) = C(b)$, which provides us with a collision for our original Pigeonhole Circuit problem. Thus, any certificate for the Erdos-Ko-Rado problem provides us with a certificate for the Pigeonhole Circuit problem above. 
	
% 	We now show that any Erdos-Ko-Rado instance must reduce to Pigeonhole Circuit. Consider an Erdos-Ko-Rado problem instance, defined by a circuit $F$ which implicitly provides us with a $2$-set system of size $2^n$. Accordingly, we define a Pigeonhole Circuit instance whose witness allows us to recover a witness for the original Erdos-Ko-Rado problem instance. To do so, we construct a circuit $C: \{0,1\}^n \mapsto \{0,1\}^n$. 
	
% 	We first arbitrarily identify two sets from the set system, $F$. Without loss of generality, we identify $F(0)$ and $F(1)$. If these two sets are disjoint, identical, or invalid, we are done. Otherwise, they have an intersection of exactly $1$ element. Let $F(0) = (a,b)$ and $F(1) = (b,c)$, such that their intersection is $\{b\}$. We now define our Pigeonhole, $C$, as follows: 
	
% 	\begin{enumerate}
% 		\item For some index $i$, if $F(i)$ outputs an invalid set, $C(i) = 0$
% 		\item For some index $i$, suppose $F(i)$ contains both $b$ and $d$ (where $d\neq{b}$), then we let $C(i) = d$.
% 		\item For some index $i$, if $F(i)$ does not contain $b$, then $C(i) = 0$. 
% 	\end{enumerate}
	
% 	We now demonstrate that a solution to the Pigeonhole Circuit problem with circuit $C$ allows us to recover a certificate to the original Erdos-Ko-Rado problem. 
	
% 	There are two cases to consider here. We start by considering the case in which we recover a zero element. That is, we find an element $x$ with $C(x) = 0$. This can only happen in $2$ cases, based on the above definition of $C$.  First, $F(x)$ might generate an invalid set. In this case, $x$ is a valid certificate. Second, $F(x)$ might not contain $b$. In this case, suppose $F(x) = (p,q)$. We note that $x$ is distinct from $1$ and $0$, because $0$ and $1$ are not zero elements, based on the above definition. If $F(x)$ is disjoint from either $F(1)$ or $F(0)$, then we are done. If, instead, $F(x)$ does not contain $b$ and has nonempty intersection with $F(1)$ and $F(0)$, then $F(x)$ must contain $a$ and $c$. Then, consider \textit{any} index $y$ that is distinct from $0,1,x$. If $F(y)$ is invalid, we are done. If $F(y)$ is identical to one of $F(0), F(1), F(x)$, we have found a repeated set certificate, and we are done. Otherwise, $F(y)$ must be fully disjoint from at least one of $F(0), F(1), F(x)$, and we can recover a disjoint set. That is, the only way a set $F(y)$ of size intersects each of $\{a,b\}, \{a,c\}, \{b,c\}$ is if $F(y)$ is identical to one of $\{a,b\}, \{a,c\}, \{b,c\}$. 
	
% 	Now,suppose that we recover a collision from $C$. That is, we find two distinct $n$-bit strings $x$ and $y$ with $C(x) = C(y)$. First, suppose $C(x) = C(y) \neq{0}$. Based on the above definition of $C$, this can only happen if $F(x)$ and $F(y)$ both contain the element $b$ as well as the element $C(x)$. In this case, $F(x)$ and $F(y)$ both describe the set $\{b, C(x)\}$, which means that we have recovered a "repeated set" certificate. In the second case, suppose $C(x) = C(y) = 0$. That is, suppose we have found two zero certificates. In this case, the argument from above tells us that we can recover the desired certificate using any one of these zero certificates.  In this case, $F(x)$ and $F(y)$ are each either invalid sets or they do not contain $b$. In the case that they are invalid sets, we are done. If these indices both do not contain $b$, then $F(x)$ and $F(y)$ must each contain both $a$ and $c$ in order to have nonempty intersection with $F(1)$ and $F(2)$. 
	
	
% \end{proof}

% \subsubsection{Generalization of Erdos-Ko-Rado to larger set-systems}

% In the above example, we called the problem $2$-Erdos-Ko-Rado because each set in the set system had size $2$. Of course, we can generalize this problem along the following lines: suppose we are given a set system in which the sets have size $k$ for some constant $k > 2$. Each element of these sets comes from a universe of size $2^n$, as above. Further, suppose that there are more than  ${2^n - 1 \choose{k-1}} + 1$ sets in the set system. By the Erdos-Ko-Rado theorem, there must be two disjoint sets (or at least one invalid set). We can, in effect, define a generalization of Erdos-Ko-Rado: 

% \begin{defi}[Problem Statement: $k$-Erdos-Ko-Rado]
% 	Consider a universe, $X$ consisting of the integers in the range $[0, 2^n - 1]$. We define a $k$-set system $S$ using a concisely represented circuit, where $|S| = {2^n-1\choose{k-1}} + 1$. In particular, 
% 	$$F: \{0,1\}^{\lceil log(|S|) \rceil} \mapsto X^k $$
% 	$F$ takes, as input, an index represented by $\lceil log(S) \rceil$-bits. It outputs $k$ elements from the universe $X$. Each element is represented by a $n$-bit string. Together, these elements form a set of size $k$. The challenge is to find one of the following: 
% 	\begin{enumerate}
% 		\item Invalid set: Find an input, $i<|S|$ such that $F(i)$ contains two identical elements.
% 		\item Repeated set: Find distinct inputs, $i, j < |S|$ such that $F(i)$ and $F(j)$ output the same set.  
% 		\item Disjoint set: Find inputs, $i, j < |S|$, such that $F(i)$ and $F(j)$ are disjoint. 
% 	\end{enumerate} 
% \end{defi}




==> Preliminaries.tex <==
\subsection*{Preliminaries}
In this section, we summarize some definitions and results which we will use repeatedly in this paper. 

\noindent
\paragraph{PPP:} In the generic problem for PPP we are given a Boolean circuit $C$ with $n$ input bits and $n$ output bits, and we seek either (a) an input $x$ such that $C(x)=0^n$, or (b) a {\em collision}, two distinct inputs $x\neq y$ such that $C(x)=C(y)$.  For the {\em weak} version of this class, PWPP, the circuit has $n$ inputs and $n-1$ outputs, and a collision is sought.  It is known that $n-2$ of fewer outputs, down to $n^\delta$ for any $\delta>0$, yield the same class, see \cite{???}.  
\paragraph{Ramsey:}

\if{false}

\begin{defi}[Problem: Pigeonhole Circuit]
	We are given a circuit $C$: 
	$$C: \{0,1\}^{n} \mapsto \{0,1\}^n $$
	The problem is to find one of the following: 
	\begin{enumerate}
		\item \textbf{Zero Element:} An element $a$ mapping to zero: $C(a) = 0$
		\item \textbf{Collision: }Two elements $a$ and $b$ such that $C(a) = C(b)$
	\end{enumerate}
\end{defi}

\begin{defi}[Weak Pigeonhole Problems PWPP(n, n-k)]
	The complexity class PWPP captures the weak pigeonhole principle, and has the following complete problem: 
	We are given a circuit $C$ with: 
	$$C: \{0,1\}^{n} \mapsto \{0,1\}^{n-k} $$
	The challenge is to find two distinct $n$-bit strings $i$ and $j$ with $C(i) = C(j)$. 
\end{defi}

A PWPP-complete problem is PWPP(n, n-1). It was proved in \citep{JERABEK2016380} that PWPP(n, n-1) is equivalent to PWPP(n, $n^{\delta}$), for any $\delta < 1$. In other words, compression by a single bit is equivalent to compression by polynomially many bits.

The following definition is from \citep{Komargodski2019}:

\begin{defi}[Collision Resistant Hash (CRH) Function Family]
	We consider families of functions $F_n = \{C: \{0,1\}^{n} \mapsto \{0,1\}^{p(n)}   \}$ for each positive integer $n$, where $n > p(n)$ and $p(n)$ is a polynomial in $n$ . We say a family $F_n$ is a collision resistant hash function family if for any probabilistic algorithm, $A$, the probability that $A$ finds a collision on a randomly sampled member of $F_n$ is arbitrarily small. 
\end{defi}

\subsection{Ramsey's Theorem and TFNP}
In this section, we summarize key results related to Ramsey's Theorem. The proofs of these results are provided, for reference, in the appendix. 

\begin{defi}[$(k, r)$-Ramsey property]
	We say a complete graph $G = (V, E)$ has the $(k,r)$-Ramsey property if there exists a coloring of its edges using $r$ colors that does not have a monochromatic clique of size $k$. 
\end{defi}

\begin{theorem}[$r$-Color Ramsey Theorem]
	Let $G = (V,E)$ be a complete graph of $r ^ {rn}$ nodes whose edges are each colored one of $r$ colors. Then $G$ has a monochromatic clique of size $n$. 
\end{theorem}

In the special case in which the number of colors is $2$ ($r = 2$), we have the $2$-color Ramsey Theorem: 

\begin{theorem}[$2$-Color Ramsey Theorem]
	Let $G = (V,E)$ be a complete graph of $2^{2n}$ nodes whose edges are each colored one of $2$ colors. Then $G$ has a monochromatic clique of size $n$. 
\end{theorem}

We now explicitly state the Ramsey problem, which was identified by \citep{GOLDBERG2018} as a \textit{rogue} problem in TFNP:

\begin{defi}[Problem: Ramsey]
	We are given a concisely represented circuit $C$ which takes as input two $2n$-bit strings, and generates an output of $0$ or $1$: 
	$$C: \{0,1\}^{2n} \Cross \{0,1\}^{2n} \mapsto \{0,1\} $$
	This graph defines a 2-coloring on a complete graph of size $2^{2n}$: each node is represented by an $n$-bit string as follows: for two nodes, represented in binary as $a$ and $b$, their edge is colored "blue" if $C(a,b) = 1$ and $C(b,a) = 1$ and "red" otherwise. The challenge is to find a monochromatic clique of $n$ nodes under this coloring.  
\end{defi}

Since $C$ defines a coloring of graph edges using $2$ colors, by Ramsey's Theorem, there must exist a monochromatic clique. Thus, this problem is guaranteed to have a witness. 

Based on the proof of the $r$-color Ramsey Theorem, we can, of course, define a "multi-color" variant of the Ramsey problem: 

\begin{defi}[Problem: $(r,n)$-color Ramsey]
	We are given a concisely represented circuit $C$ which takes as input two $rn\lceil log(r)\rceil$-bit strings, and generates an output of one of $r$ colors: 
	$$C: \{0,1\}^{rn\lceil log(r)\rceil } \Cross \{0,1\}^{rn\lceil log(r) \rceil} \mapsto \{0,1\}^{log(r)} $$
	Analogous to the standard Ramsey problem, this graph defines a $k$-coloring on a complete graph of size at least $r^{rn}$. For two nodes, represented in binary as $a$ and $b$ with $a<b$, their edge is assigned color $C(a,b)$. The challenge is to find a monochromatic clique of $n$ nodes under this coloring.  
\end{defi}
\fi

==> Ramsey.tex <==
\section{Long Choice and r-Color Ramsey}
Ramsey's theorem for multi-colored graphs states that for every number $r \geq 2$ of colors and every integer $n \geq 2$, there is a number $R(r,n)$ such that for every $r$-coloring of the edges of the complete graph on $R(r,n)$ nodes there is a monochromatic clique with $n$ nodes.   The standard Ramsey theorem corresponds to the case of $r=2$ colors.  A simple proof of the multi-colored Ramsey theorem uses the same type of iterative process as the $r=2$ case, except that in every step we partition the set of available nodes into $r$ groups instead of 2\footnote{Along the same lines, we could extend Long Choice to allow the functions $P_i$ to have a more general range $[r]$ instead of $\{0,1\}$.}; as before, we pick the largest group to continue the process. 
The bound on $R(r,n)$ from this simple proof is $R(r,n) \leq r^{rn}$. Obtaining better upper and lower bounds on $R(r,n)$ for $r=2$ and for general $r$ has been (and continues to be) the subject of a long line of intense research effort.

In the computational version of the problem, denoted {\sc $(r,n)$-Ramsey}, we are given the $r$-coloring of an exponentially large complete graph, which is specified via a poly-size circuit $C$, and are asked to find a monochromatic clique of size $n$.  The {\sc Ramsey} problem of the last section is equivalent to {\sc $(2,n)$-Ramsey}.
The number $r$ of colors in general need not be fixed, it could be a function of $n$.
Assume for simplicity that $r$ is power of 2 (otherwise, replace $\log r$ in the following by $\lceil \log r \rceil$).
Every node of the complete graph is represented by a unique $rn \log r$-bit string, and the given circuit $C$ takes as input two  $rn \log r$-bit strings (two nodes $u,v$) and outputs a $\log r$-bit string (the color of the edge $(u,v)$).

\begin{theorem}
	{\sc $(r,n)$-Ramsey} is in PLC for all $r, n$.
	In particular, {\sc $(r,n)$-Ramsey} reduces to {\sc Binary Long Choice}.
\end{theorem}


\noindent
{\em Proof Sketch:} We describe first the proof for the case $r=2$, which simply follows the existence proof sketched in the previous section:
Given a 2-colored complete graph on $2^{2n}$ nodes, specified by a given circuit $C$, define the predicate $P_i$ for each $i$, to map any sequence $a_0, \ldots, a_i, x$ of nodes to the color, 0 or 1, of the edge $(a_i,x)$. Note that $P_i$ depends only on the last two arguments $a_i,x$.
Consider a valid certificate $a_0, \ldots, a_{2n}$ of this instance of Binary Long Choice.
For each $i =0, \ldots, 2n-2$, all edges $(a_i,a_j)$ for $j>i$ must have the same color, 0 or 1; assign this color to node $a_i$. At least $n$ of the $2n-1$ nodes $a_0, \ldots a_{2n-2}$ are assigned the same color.
These nodes induce a monochromatic clique of size $n$.

In the case of general $r$, given an $r$-colored
complete graph on $2^{rn \log r}$ nodes, define each function $P_i$ as follows.
Let $k= (\lfloor i/ \log r \rfloor) \log r$,
i.e, $k$ is the greatest multiple of $\log r$ that is $\leq i$.
Set $P_i(a_0, \ldots, a_i,x)$ to be the $(i-k+1)$-th bit of the color of the edge $(a_k,x)$.
Note that again all these predicates depend only on two arguments, $a_k$ and $x$. 

Consider a valid certificate $a_0, \ldots, a_{rn \log r}$ of this instance of Long Choice,
and let $b_i = a_{i \log r}$ for each $i$.
From the construction of the Long Choice instance,
it is easy to see that,
for each $i=0, \ldots , r(n-1)$, all edges $(b_i,b_j)$
for $j>i$ must have the same color:
note that the $t$-th bit of the color of edge $(b_i,b_j)$, for all $j>i$, is the value of $P_{l}(a_0, \ldots, a_l, b_j) = P_{l}(a_0, \ldots, a_l, a_{l+1})$ for $l= i \log r +t-1$.
Assign to each node $b_i$ the (common) color of the edges $(b_i,b_j)$, $j>i$.
There are $r(n-1) +1$ distinct nodes $b_0, \ldots, b_{r(n-1)}$,
each assigned one of $r$ colors, therefore at least $n$
of them are assigned the same color.
These nodes induce a monochromatic clique of size $n$.
\qed

\medskip

\if{false}
In this section, we study the relation of Ramsey-type problems to PLC. We begin by providing a general reduction from the $r$-color Ramsey problem to Long Choice. 

\begin{theorem}
	$(r,n)$-Color Ramsey is in PLC.
\end{theorem}


\begin{proof}
Suppose we are given an instance of the $(r,n)$-Color Ramsey problem ($r \geq{2}$). This instance is defined by a poly(n)-sized circuit, $C$:
	
$$C: \{0,1\}^{rn\lceil log(r)\rceil } \Cross \{0,1\}^{rn\lceil log(r) \rceil} \mapsto \{0,1\}^{log(r)} $$
	
	This circuit defines a coloring of the edges of a complete graph, $G$, consisting of $2^{rn\lceil log(r)\rceil }$ nodes. Each vertex is represented by a unique $rn\lceil log(r)\rceil$-bit string. Each edge is assigned one of $r$ colors, where each color is represented by a unique $log(r)$-bit string.
	
	To reduce this problem to Long Choice, it suffices to define the predicate functions $P_0,$ $\dots$,$ P_{rn\lceil log(r)\rceil - 2}$. We will define these predicate functions in such a way that the first $k = r(n-1)\lceil{log(r)}\rceil + 1$ elements of any valid Long Choice certificate are sufficient to recover a monochromatic clique for the Ramsey problem. By the definition of Long Choice, the first $k$ elements are only constrained by the first $k-1$ predicate functions. Therefore, we carefully define the predicate functions $P_i$ for $i \leq{k-2}$. Furthermore, whenever $i \leq{k-2}$, we define $P_i$ whenever its input consists of distinct elements $a_0, a_1, \ldots, a_{i}, a_{i+1}$ (the case in which any two elements are identical is irrelevant because Long Choice requires distinct elements). For all the other predicate functions $P_j$ ($j > k-2$), we arbitrarily say that $P_j$ outputs $1$ regardless of its input because the behavior of these functions is unimportant.
	
	Consider a sequence of distinct inputs $a_0, a_1, \dots, a_i, a_{i+1}$. On such input, the function $P_i$ does the following:
	
	\begin{enumerate}
	    \item Let $x$ be the largest multiple of $\lceil log(r) \rceil$ strictly less than $i+1$.
	    \item Let $p$ denote $(i+1) - x$. $P_i$ returns the $p$-th bit of $C(a_x, a_{i+1})$. 
	\end{enumerate}
	
	Based on this definition, consider any valid Long Choice certificate, given by the sequence $a_0, \dots, a_{rn\lceil log(r) \rceil}$. In particular, consider the subsequence $b_0, b_1, \dots, b_{r(n-1)}$, where $b_i = a_{i * \lceil log(r) \rceil}$. These elements have the following property: for any fixed $x < r(n-1)$, $C(b_x, b_y)$ is the same value for all $y > x$. This condition is enforced by the predicate functions $P_{x}, \dots, P_{x + \lceil log(r) \rceil -1}$. To see why, note that for every $b_y$, 
	
	
	$$P_{x*\lceil log(r) \rceil}(a_0, a_1, \dots, a_{x*\lceil log(r) \rceil-1}, b_x, b_y) = P_{x*\lceil log(r) \rceil}(a_0, a_1, \dots, a_{x*\lceil log(r) \rceil-1}, b_x, a_{x*\lceil log(r) \rceil+1})$$
	
	Furthermore, these two expressions return the first bits of $C(b_x, b_y)$ and $C(b_x, a_{x*\lceil log(r) \rceil+1})$, respectively. Therefore, the first bit of $C(b_x, b_y)$ is must always be equal to the first bit of $C(a_{x*\lceil log(r) \rceil}, a_{x*\lceil log(r) \rceil+1})$. We can use the same argument with predicate function $P_{x*\lceil log(r) \rceil+1}$ to argue that the \textit{second} bit of $C(a_{x*\lceil log(r) \rceil}, a_{x*\lceil log(r) \rceil+2})$ must equal the second bit of $C(b_x, b_y)$. More generally, we can use this exact argument to show that $C(b_x, b_y)$ must agree on all bits for all $b_y$, which means that node $b_x$ has monochromatic edges with all $b_y$ ($y > x$). 
	
	We can therefore assign a color to each element as follows: for every $i < r(n-1)$, $b_i$ is assigned the color $C(b_i, b_{i+1})$; we arbitrarily assign $b_{r(n-1)}$ one of the $r$ colors in the graph. 
	
	There are $r(n-1) + 1$ elements in this sequence, and each element has been assigned one of $r$ colors. Therefore, by the pigeonhole principle, there must exist at least $n$ elements with the same color; call these elements $b_{i_0}, b_{i_1}, \dots, b_{i_n}$, where $i_0 < i_1< \dots < i_n$. Since each of these nodes has been assigned the same color, we know that the edges between each pair of nodes is the same color. Therefore, these elements for our monochromatic clique. This completes the proof. 
\end{proof}

In the special case that the number of colors, $r$, is $2$, we find that all predicate functions only need their last two inputs. In that case, we can therefore conclude that $(2,n)$-Ramsey reduces to Binary Long Choice. 

\begin{theorem}
	$(2,n)$-Ramsey Reduces to Binary Long Choice
\end{theorem}

\fi

Finally, consider how Ramsey relates to PWPP. It was shown previously in \citep{Komargodski2019} that there exists a randomized reduction from PWPP to {\sc Ramsey},  as well as a deterministic reductions from PWPP to the multi-color Ramsey problem. In the appendix, we use properties of metric spaces to provide an alternative deterministic reduction from PWPP to multi-color Ramsey.


% \subsection{PWPP-hardness of Ramsey variants}
% One striking commonality between Ramsey type problems and PWPP is that both problems have exponentially many valid certificates. Furthermore it is shown in previous work that there exists a randomized reduction from PWPP to Ramsey \citep{Komargodski2019} as well as deterministic reductions between PWPP and multi-color Ramsey problems. In this section we describe a series of reductions from PWPP to variants of the Ramsey problem. Our reduction makes use of properties of metric spaces. We start with relevant background.

% \begin{theorem}
% 	Any collection of pairwise equidistant points in $\mathbb{R}^n$ cannot have size greater than $n + 1$.
% \end{theorem}

% The above result uses the standard Euclidean distance metric in $\mathbb{R}^n$. Consider the set $U = \{0,1\}^m$. Note that the Hamming and Euclidean distance metrics are in direct correspondence over $U$. In particular, the Hamming distance between two elements $i, j\in {U}$ is the \textit{square} of the Euclidean distance between those two elements. This leads to the following observation: 

% \begin{theorem}
% 	Consider the set $U= \{0,1\}^m$. There cannot be more than $m+1$ pairwise equidistant points in $U$, where distance is measured using the Hamming distance metric.
% \end{theorem}


% Recall that we can reduce any problem instance of PWPP(n, n-1) to a problem instance of PWPP(n, $n^{\delta}$), for some constant $0 < \delta < 1$. 

% We now define the multi-color Ramsey problem more precisely. In the following discussion, we omit the use of floor and ceiling functions to make things more readable. 

% \begin{defi}[$k$-color standard Ramsey]
% 	We are given a graph of $2^n$ nodes, each represented by a unique $n$-bit string. We are given a concisely represented circuit, $C$, which takes as inputs two distinct nodes and outputs their color: 
	
% 	$$C: \{0, 1\}^n \mapsto \{0,1\}^{log(k)} $$
	
% 	The challenge is to find a monochromatic clique of size $\frac{n}{k*log(k)}$. Such a clique is guaranteed to exist by Ramsey's Theorem  
% \end{defi}

% \begin{defi}[$k$-color standard Ramsey]
%     This is shorthand notation for a $(k, \frac{n}{k*log(k)})$-color Ramsey problem. Note that this problem is defined on a graph of size $2^n$; this is why we call it a standard problem. 
% \end{defi}

% First note that this problem definition is just a restatement of the original $(k, n)$-color Ramsey problem; we are just fixing the size of the graph. Put differently, we can express a $k$-color standard Ramsey problem as a $(k, n)$-color Ramsey problem by changing $n$ appropriately. 
% We can relate these problems to PWPP as follows: 

%\begin{theorem}
%	$(n^{\delta})$-color standard Ramsey is PWPP-hard whenever $\delta < 1/2$
%\end{theorem}

% \begin{proof}
% 	Fix any positive $\delta < 1/2$. Consider a PWPP-complete problem, $A$. As mentioned above, since compression by a single bit is equivalent to compression by polynomially many bits, we can reduce $A$ to a PWPP(n, $n^{\delta}$) problem. This problem is defined by a circuit, $C$: 
	
% 	$$C: \{0,1\}^{n} \mapsto \{0,1\}^{n^{\delta}} $$
	
% 	We reduce this problem to a $n^{\delta}$-color standard Ramsey problem, which is defined by a circuit: 
	
% 	$$C_r: (\{0, 1\}^n)^2 \mapsto [n^{\delta}]$$
	
% 	$C_r$ is defined as follows: for distinct inputs, $i, j$, $C_r$: 
% 	\begin{enumerate}
% 		\item Returns the hamming distance between $C(i)$ and $C(j)$ if $C(i) \neq{C_j}$
% 		\item Returns $\lceil n^{\delta} / 2 \rceil$ if $C(i) = C(j)$. 
% 	\end{enumerate}

% 	As mentioned above, this problem is total and we are guaranteed to find a clique of size $\frac{n}{\delta * log(n) * n^{\delta}} = \frac{n^{1-\delta}}{\delta * log(n)} \geq{\frac{n^{1 - \delta }}{\delta * n^{\epsilon}}} > 2 * n^{\delta}$, where $0<\epsilon<1/2 - \delta$ and all inequalities hold asymptotically. Thus, the guaranteed clique size is greater than $n^{\delta} + 1$. 
	
% 	We know that there are at most $n^{\delta} + 1$ distinct points in $\{0,1\}^{n^{\delta}}$ which are pairwise equidistant (under hamming distance). 
% 	Consider a desired certificate (a clique) consisting of vertices $a_1, a_2, \dots, a_i$. What is the color of the edges of this clique? We claim that it must be the color $\lceil n^{\delta} / 2 \rceil$. To see why, suppose that it is any other color. Then, consider the $n^{\delta}$-bit strings $C(a_1), C(a_2), \dots, C(a_i)$. By the definition of $C_r$, this collection of values must be pairwise equidistant, which is impossible since $i > n^{\delta} + 1$.
	
% 	Thus, $C_r(a_x, a_y) = \lceil n^{\delta} / 2 \rceil$ for all $a_x, a_y$. Furthermore, there can be at most $n^{\delta} + 1$ distinct elements in the set $C(a_1), C(a_2), C(a_3), \dots, C(a_i)$. Thus, at least two elements of our clique collide under $C$, and we are done. 
% \end{proof}






==> Schur.tex <==
\section{Schur's Theorem in TFNP}

Schur's Theorem is another result from extremal combinatorics whose proof employs an iterated application of the Pigeonhole Principle. There are two upper bounds which we will discuss. We refer the reader to \citep{jukna} for a more detailed discussion. The weaker bound is a direct application of Ramsey's Theorem; its proof can be found in \citep{graham1990ramsey}. The stronger bound iteratively applies a Pigeonhole Principle argument. This proof can be found in \citep{jukna}. We include this exact proof here for reference. For each of these bounds, we can formulate a unique TFNP problem. Then, we study the relation between the Schur problem and Long Choice. 


\begin{theorem}[Schur's Ramsey Theorem]
	For any coloring of the first $2^{2rlog(r)}$ positive integers using $r$ colors, there exists monochromatic $a$, $b$, and $a + b$. 
\end{theorem}

\begin{proof}
	To prove the above statement, we start with some coloring of the first $2^{2rlog(r)}$ positive integers. That is, we are given some function $f$: 
	
	$$f: [2^{2rlog(r)}] \mapsto [r] $$
	
	which maps each integer to a single color.% Each color is represented exactly one of the integers in the set $[r]$. 
	Accordingly, we construct a complete graph, $G = (V, E)$, with a vertex set consisting of $2^{2rlog(r)}$ vertices. We arbitrarily number these vertices $1, 2, \dots, 2^{2rlog(r)}$. We can define a coloring of the edges of this graph as follows: for two vertices, numbered by $x$ and $y$ (with $x < y$), the color of edge $(x, y)$ is defined to be $f(y - x)$. By the $r$-color Ramsey Theorem, this graph must contain a monochromatic triangle. Suppose the vertices of this triangle were assigned numbers $a < b < c$. Then, by definition, $f(c - b) = f(c - a) = f(b - a)$. But $(b - a) + (c - b) = (c - a)$. This completes the proof. 
\end{proof}

There exists a TFNP search problem based on this theorem:

\begin{defi}[Weak Schur]
	We are given a concisely-represented circuit, $C$, which implicitly defines a coloring on the first $2^{2rlog(r)}$ integers that uses $r$ colors:
	
	$$C: \{0,1\}^{2rlog(r)} \mapsto \{0,1\}^{log(r)}  $$
	
	For any integer, $i$, in the interval $[2^{2rlog(r)}]$, the circuit takes as input the binary representation of $i - 1$. This input can (by definition) be encoded by a $2rlog(r)$-bit string. Accordingly, $C(i)$ returns the color of the integer $i$. 
	
	The Weak Schur problem asks to return two (not necessarily distinct) inputs $a$ and $b$ with $C(a) = C(b) = C(a+b)$.
\end{defi}

Based on the proof, we can conclude that the Weak Schur problem reduces to $(r, 3)$-Ramsey, which, as discussed above, is in PLC.

\begin{theorem}
    Weak Schur is in PLC.
\end{theorem}

In addition Schur's Ramsey Theorem, there is a stronger bound which involves an iterative application of the Pigeonhole Principle. 

\begin{theorem}[Schur's Theorem]
	For any coloring of the first $\lceil e * r! \rceil$ integers using $r$ colors, there exists three monochromatic integers $x, y, z$ with $x + y = z$.
\end{theorem}	

For a detailed proof, see \citep{jukna}.


Of course, the only difference between the two problems is their extremal bounds: strong Schur has a smaller extremal bound than weak Schur. Therefore, we have the following natural relation:

\begin{theorem}
    Weak Schur is polynomially reducible to Strong Schur.
\end{theorem}

\begin{proof}
    A problem instance of Weak Schur specifices a coloring over the first $2^{2rlog(r)}$ positive integers, given by a circuit, $C$. We can define a new circuit $C'$ which only colors the first $2^{rlog(r) + 2}$ in exactly the same fashion as $C$. The circuit $C'$ fully specifies a Strong Schur problem, and a valid certificate to that problem is also a valid certificate to the original Weak Schur problem instance. 
\end{proof}

\subsubsection{Average-Case Hardness of Schur 
<To Do, if solution exists here..>
% We now show that the Strong Schur problem has average-case hardness properties under standard cryptographic assumptions (specifically, assuming Collision Resistant Hash Functions exist). This answers a question posed in \citep{Komargodski2019}. To do this, it suffices to argue that the Weak Schur problem has these average-case hardness properties. 

% We begin by describing an explicit construction of a Schur-free coloring: that is, a coloring over the first $k$ positive integers with the property that there is \textit{no} monochromatic $a$, $b$, and $a+b$. This construction is described in \citep{Schur1916}.

% \begin{theorem}
% 	There exists a coloring of the first $3^{r-1}$ integers using $r$ colors which does not contain any monochromatic elements $x$, $y$, and $x + y$. Furthermore, this coloring can be represented concisely by a circuit. 
% \end{theorem}

% \begin{proof}
% 	We provide a construction inductively.  Suppose that there is a coloring of the first $n$ positive integers using $r$ colors that does \textit{not} contain any monochromatic elements $x$, $y$, and $x + y$. This coloring is essentially a function $f_1$: 
	
% 	$$f_1: [n] \mapsto [r] $$
	
% 	We argue there exists a coloring, $f_2$ of the first $3n$ positive integers using $r + 1$ colors with the same property. We have: 
	
% 	$$f_2: [3n] \mapsto [r+1] $$
	
% 	For any input $i\in{[3n]}$, we define $f_2(i)$ on a case-by-case basis: 
	
% 	\begin{enumerate}
% 		\item If $i\leq{n}$, we let $f_2(i) = f_1(i)$
% 		\item If $n < i \leq{2n}$, we let $f_2(i) = r+1$
% 		\item If $n > 2n$, we let $f_2(i) = f_1(i - 2n)$
% 	\end{enumerate}
	
% 	It remains to prove that this coloring also has the property that there are no monochromatic $x$, $y$, and $x + y$. Suppose, without loss of generality, that $x < y$. We have three cases to consider: 
	
% 	\begin{enumerate}
% 		\item Case 1: $x \leq{n}$. First, suppose that $y\leq{n}$. We know that the coloring $f_2$ agrees with $f_1$ over the interval. By assumption, there are no $x, y \leq{n}$ with $x$, $y$, $x+y$ monochromatic. Next, suppose that $n < y \leq{2n}$. In this case, $f_2(y) = r+1$, while $f_2(x) < r + 1$, so $x$ and $y$ cannot be monochromatic. Third, suppose $y > 2n$. Further, suppose $x$, $y$, and $x + y$ are monochromatic. Since $y, x + y > 2n$, we know that $f_2(y) = f_1(y - 2n)$ and $f_2(x+y) = f_1(x+y - 2n)$. But note that $y - 2n < n$ and $ x + y - 2n < n$. Since $(x) + (y-2n)= (x + y - 2n)$, this would mean there exists $a, b, c < n$ with $a + b = c$ and $f_1(a) = f_1(b) = f_1(c)$, contradiction. 
% 		\item Case 2: $n < x \leq{2n}$. In this case, the only elements $y$ colored the same way as $x$ are those $y$ with $n < y \leq{2n}$. In particular, we must have $f_2(x) = f_2(y) = r + 1$. But since $n < x\leq{2n}$ and $n < y \leq{2n}$, we know $ x + y > 2n$. Thus, $f_2(x+y) = f_1(x + y - 2n) < r + 1$. Therefore, there are no monochromatic $x$, $y$, $x + y$. 
% 		\item Case 3: $2n < x \leq{3n}$. Consider any element $y$. In this case, we would need $ y<n$ (otherwise, $x + y > 3n$). Suppose that $x$, $y$, and $x + y$ are monochromatic. Since $ 2n < x < x + y$, we know that $f_2(x) = f_1(x - 2n)$ and $f_2(x + y) = f_1(x + y - 2n)$. Note that $x - 2n, x + y - 2n$, and $y$ are all less than $n$, and $x - 2n + y = x + y - 2n$. Since $f_1(x-2n) = f_1(y) = f_1(x + y - 2n)$ by our assumption, this means we have found $a b < n$ with $a$, $b$, $a + b$ monochromatic, contradiction. 
% 	\end{enumerate}
	
% 	Thus we have shown that $f_2$ does provide the desired coloring. If we want to create a coloring using $r$ colors, we can repeatedly apply the above argument up to $r - 1$ times. 
	
% 	Namely, we start with a coloring of the set $[1]$ with $1$ color. This trivially satisfies the desired property. We then iteratively apply the above construction $r - 1$ times. This yields the desired coloring on the first $3^{r-1}$ integers using $r$ colors.
	
	
% 	It now remains to show that the above coloring can be concisely represented by a circuit, $C$. This circuit takes, as input, the binary representation of an integer in the interval $[3^{r-1}]$. It returns this integers' corresponding coloring, represented by a binary string of $log(r)$ bits. We now explain, algorithmically, how the circuit $C$ will define the coloring described above. It is first useful to note that in the above construction, we apply an "extension" step iteratively ($r-1$ times). In particular, given a coloring, $f_i$, over the first $n$ integers, we show how to define a new coloring, $f_{i+1}$, over the first $3n$ integers. The reason we call this operation an extension is that $f_i$ and $f_{i+1}$ agree over $[n]$, the domain of $f_i$. In this sense, $f_{i+1}$ extends $f_i$. 
	
% 	By the nature of this construction, we can show, inductively, that the whole coloring can be represented concisely by a circuit. 
	
% 	As a base case, we specify an arbitrary coloring of the singleton set, $\{1\}$. This coloring uses only one color. 
	
% 	Now, we assume that $f_i$, a coloring over the first $n$ integers using $r$ colors, can be represented efficiently as an integer.  
	
% 	Based on this assumption, we now show that $f_{i+1}$, a coloring over the first $3n$ integers using $r+1$ colors, can also be represented concisely by a circuit. In particular, if we suppose $f_{i+1}$ is given, as input, an integer $k$, then:
	
% 	\begin{enumerate}
% 		\item If $k$ lies in the domain of $f_{i}$, $f_{i+1}$ returns $f_{i}(k)$.
% 		\item If $k$ lies in the interval $[n+1, 2n]$, then $f_{i+1}(k) = r+1$
% 		\item If $k$ lies in the interval $[2n+1, 3n]$ then $f_{i+1}(k) = f_i(k - 2n)$.
% 	\end{enumerate}
	
% 	We note that all of these conditions can be efficiently evaluated (by our assumption). The definition of these functions exactly mirrors the definitions of the colorings from the construction above. As in our construction, we can apply this argument iteratively $r-1$ times to conclude that we represent the whole coloring efficiently. 
% \end{proof}



==> ShortChoice.tex <==
\section{Short Choice}

As we have seen above, PPP is contained in the class PLC. There is an intuitive reason for this: implicit in any PPP-complete problem is an iterated pigeonhole argument.

% Consider a pigeonhole circuit problem, given by a poly(n)-sized circuit, $C$:

% $$C: [2^n + 1] \mapsto [2^n] $$

% where the inputs and outputs are represented concisely using $O(n)$ bits, and the challenge here is to find a collision. We can use the following standard argument: there must exist a bit, $c_1$, such that the majority of the elements in the domain of $C$ map to a string whose first bit is $c_1$. By the pigeonhole principle, there must be at least $2^{n-1} + 1$ elements whose first bit is $c_1$. Amongst these elements, there must exist a bit $c_2$ such that at least half of these elements map to a bit string whose second bit is equal to $c_2$; that makes for at least $2^{n-2} + 1$ elements. If we continue this argument a total of $n$ times, we can conclude that there must be at least two elements which have all bits of their image under $C$ in common. These two elements represent a collision under $C$.  

% In the above discussion, we have repeatedly used a majority argument: if we partition $k$ objects into 2 classes, one class must have at least $k/2$ objects by the pigeonhole principle. 

The class PEPP, introduced in \citep{Kleinberg2020TFNP}, embodies the dual of the class PPP - an anti-pigeonhole principle: if there are $2^n - 1$ pigeons and $2^n$ holes, then no matter how the pigeons are placed, there must be an empty hole. PEPP belongs to the class \textbf{TF$\Sigma_{2}$P}, which is believed to lie outside of the class $NP$.

While the existence proof for Pigeonhole Circuit has a majority argument, the existence proof for Empty has a corresponding ``minority" argument. Suppose we are given an instance of the PEPP-complete problem \textit{EMPTY}: we are given a poly(n)-sized circuit $C: [2^n - 1] \mapsto [2^n] $,
where the inputs and outputs are all represented concisely using exactly $n$ bits. The challenge here is to find an element $j$ in the range such that there is no $i$ with $C(i) = j$. There must exist a bit $c_1$ such that the minority of elements in the domain of $C$ map to a $n$-bit string whose first bit is $c_1$. This minority has size \textit{at most} $2^{n-1} - 1$. Among the elements in this minority, there must exist a bit $c_2$ such that the minority of these elements map to a $n$-bit string whose second element is $c_2$. This new minority has size \textit{at most} $2^{n-2} - 1$. If we continue this argument $n$ times, we find that there exists a bit string $c_1 \circ c_2 \circ \dots \circ c_n$ which is not in the image of $C$.

As discussed earlier, {\sc Long Choice} is a generalization of PPP that encapsulates the iterated majority arguments. We can define an analogous generalization of the class PEPP that encapsulates the iterated minority argument. For this, we introduce a problem called {\sc Short Choice}, a problem in \textbf{TF$\Sigma_{2}$P} which is the dual of {\sc Long Choice}. 

\begin{defi}[Subcertificate]
    Given a Long Choice problem instance defined by predicate functions $P_0, P_1, \dots, P_{n-2}$ we call a subcertificate a sequence of distinct elements $a_0, a_1, \dots, a_k$ ($k \leq n$) which satisfy the {\sc Long Choice} conditions imposed by the predicate functions $P_i$. That is, for each predicate function $i < k$, we require that $P_i(a_0, \dots a_{i}, a_j) $ 
    is the same for all $j > i$. 
\end{defi}

\begin{defi}[Problem: {\sc Short Choice}]
	The input is the same as in the {\sc Long Choice} problem, except that the universe $U$ has  now $2^n - 2$ objects. As in {\sc Long Choice}, we are given a sequence of $n-1$ poly($n$)-sized circuits, $P_0, \dots, P_{n-2}$, where each $P_i$ defines a predicate function $ P_i : U^{i+2} \mapsto \{0,1\}$ 
	
	The problem is to find  a sequence $a_0, a_1, \dots, a_{k}$ of $k \leq n-1$ distinct objects in $U$ and a bit $c \in \{0, 1\}$ with the property that (1) the sequence $a_0, a_1, \dots, a_{k}$ is a subcertificate, and (2)  there does not exist any object $a_{k+1} \in U$ that both extends this subcertificate and has $P_{i}(a_0, a_1, \dots, a_{i}, a_{k+1}) = c$. 
\end{defi}

As in our discussion of {\sc Long Choice}, we can show that {\sc Short Choice} is both total and PEPP-hard. The proof of totality uses a repeated minority argument, in the same way that the proof for Long Choice used a repeated majority argument. And the proof of PEPP-hardness is along similar lines as the PPP-hardness proof for {\sc Long Choice}. We provide the complete proofs in the appendix. 

\begin{theorem}
    {\sc Short Choice} is a total problem.
\end{theorem}

% \begin{proof}
%     Let $U$ denote the set of $2^n - 2$ objects in the universe of this Short Choice problem instance. We will construct a certificate, given by a Long Choice subsequence $a_0, a_1, \dots, a_{k}$, $(k \leq{n-2})$ and a bit $c$. In order to construct this sequence, we will also define a sequence of nonempty sets $U_0 \supset U_1 \supset \dots \supset U_{k}$ with the following properties: 
%     \begin{enumerate}
%         \item $U_0 = U$
%         \item $|U_k| \leq 2^{n - k} - 2$ for all $k$
%         \item $a_k \in U_k$ for all $k$ \textit{and} whenever $k\geq{1}$, $a_0, \dots, a_{k-1} \not\in U_{k}$.
%         \item For every $j \leq k$, the element $x$ extends the Long Choice subcertificate $a_0, a_1, \dots, a_j$ if and only if $x\in U_j \setminus \{a_j \}$. 
%         \item For any $x\in{U_{j+1}}$, $P_j(a_0, \dots, a_{j}, x)$ is constant.
        
%     \end{enumerate}
    
%     As a base case, we begin by defining $U_0 := U$, and we pick an arbitrary element $a_0\in{U_0}$. Note that the base case of our construction so far satisfies properties $1$ and $2$: $U_0 = U$, $|U_0| = |U| \leq 2^{n - 0} - 2$. Property $3$ holds because $a_0 \in U_0$ (the second condition in property $3$ is vacuously true here). Property $4$ holds trivially, since any element $x \neq a_0$ must belong to $U_0 \setminus a_0$. 
    
%     We now define $U_1$ in such a way that our base case satisfies property $5$ as well. We partition the elements $x\in \{U_0\setminus{ \{a_0 \}  } \}$ in two groups based on the value $P_0(a_0, x)$. We know that $|U_0\setminus{ \{a_0 \}  }| = 2^n - 3 $, and since this set is being partitioned into two disjoint sets, the minority must have size at most $2^{n-1} - 2$. If the minority is nonempty, we define $U_1$ to be the minority (which guarantees condition $5$ holds). We also define $a_{1}$ as an arbitary element of $U_1$. Otherwise, if the minority is empty, this means that $P_0(a_0, x)$ takes on a constant value (call it $c$) for all $x\in U\setminus \{a_0 \}$. This in turn means that there is no value $x$ with $P_0(a_0, x) = \neg c$ (the oppose of bit $c$). We can thus return $a_0$ along with the bit $\neg c$ as a valid certificate to the Short Choice problem. This completes the base case. 
    
%     Now, suppose for some $0 \leq j \leq {k}$ we have defined the nonempty sets $U_0 \supset U_1 \supset \dots \supset U_j$ and the subsequence $a_0, a_1, \dots, a_{j}$ in such a way that they satisfy the above properties. We can first conclude based on properties $3$ and $5$ that the sequence $a_0, \dots, a_j$ is a valid Long Choice subcertificate. Furthermore, an element $x$ extends this Long Choice subcertificate if and only if it belongs to $U_j\setminus \{ a_j \}$, according to property $4$.
    
    
    
%     % To see why, first suppose that $x \in U_j\setminus \{ a_j \}$. This implies $x \in U_k$ for all $k \leq j$. Then, by property $4$, $P_k(a_0, \dots, a_{k}, a_{k+1}) = P_k(a_0, \dots, a_{k}, x)$, for every $k < j-1$, so $x$ extends the certificate. 
    
%     % To prove the converse, assume that $x$ extends the certificate, but $x \not\in U_j \setminus \{a_j\}$. Since $U_0 = U$, it is certainly true that $x\in U_0$. Consider the largest nonnegative integer $i$ such that $x \in U_i$. Then, by definition, $x \not\in U_{i+1}$, but $a_{i+1}\in U_{i+1}$ from our inductive hypothesis. Then, by definition of the sets $U_0, \dots, U_k$, 
    
%     % $$P_{i+1}(a_0, \dots, a_{i+1}) \neq P_{i+1}(a_0, \dots, a_i, x)$$
    
%     % Therefore, $x$ cannot extend the certificate, contradiction. 
    
%     To continue our inductive construction, we partition the elements $x\in \{ U_j \setminus \{a_j \} \}$ based on the the value of $P_j(a_0, \dots, a_j, x)$. If one side of this partition is empty, that means that there exists a bit $c\in{ \{0, 1\} }$ such that there are no elements $x\in \{ U_j \setminus \{a_j \} \}$ where $a_0, a_1, \dots, x$ is a Long Choice subcertificate and $P_j(a_0, \dots, a_j, x) = c$. In this case, we are done: the sequence $a_0, \dots, a_j$ along with the bit value $c$, serves as a certificate to the problem. 
    
%     Otherwise, both sides of this partition are nonempty. In this case, we can continue the inductive construction: we pick the minority side of the partition of the elements $x\in \{ U_j \setminus \{a_j \} \}$. We then define $U_{j+1}$ to be all of the elements on the minority side of the partition, and pick an arbitrary element $a_{j+1}\in{U_{j+1}}$ to extend the Long Choice subsequence. We know by the inductive hypothesis that $|U_j| \leq 2^{n -j} - 2$, and by the same Pigeonhole argument used in the base case, we know that $|U_{j+1}| \leq 2^{n -j} - 2$, as desired. Thus properties $1$ and $2$ hold. To see why property $3$ holds, note that $a_{j+1} \in U_{j+1}$. Furthermore, $a_0, \dots, a_{j-1} \not\in U_j \supset U_{j+1}$. Finally, $a_j \not\in U_j$, as stated above. To see why property $4$ must hold, consider any candidate element $a_{j+2}$ which may extend the Long Choice subcertificate. We know from the inductive hypothesis that $a_{j+2}$ must belong to $U_j \setminus a_j$. Additionally, we must also now have have that 
    
    
%     $$P_j(a_0, \dots, a_j, a_{j+1}) = P_j(a_0, \dots, a_{j}, a_{j+2})$$
    
%     By the definition of $P_j$, this means that $a_{j+1}$ and $a_{j+2}$ both belong to $U_{j+1}$, and since $a_{j+1}$ and $a_{j+2}$ must be distinct in order to be in the same Long Choice subcertificate, we conclude $a_{j+2}\in U_{j+1}\setminus a_{j+1}$. This argument also shows that property $5$ continues to hold as well. 
    
%     Note that our construction can only proceed until $j = n-2$. To see why, suppose that $j = n-2$. Then, by our inductive hypotheses, $|U_j| \leq 2^{n-(n-2)} - 2 = 2$. Furthermore, since $a_j \in U_j$ by our assumption, we know that $U_j \setminus \{ a_j \}$ has at most $1$ other element. Denote this element (if it even exists) by $a_{n-1}$, and consider the value $c_{bad} = P_{n-2}(a_0, \dots, a_{n-2}, a_{n-1})$. It is clear that if we consider $c$ to be the opposite bit of $c_{bad}$, there are no elements $a_{i}$ which extend this Long Choice sequence with $P_{n-2}(a_0, \dots, a_{n-2}, a_{i}) = c$. Thus, we can return $a_0, \dots, a_{n-1}$ and $c$ and we are done. 
    
%     Therefore, our construction is guaranteed to terminate with a Long Choice subcertificate $a_0, \dots, a_j$ of the appropriate length, as well as a bit $c$, which provide us with a solution to the Short Choice problem.  
%     % If, however, $j = n-2$, then we can directly recover a valid certificate to this problem. To see how, first note that $|U_j| \leq 2^{n-(n-2)} - 2 = 2$ by our inductive hypothesis. Furthermore, since $a_j \in U_j$ by our assumption, we know that $U_j \setminus \{ a_j \}$ has at most $1$ other element. Denote this element (if it even exists) by $a_{n-1}$, and consider the value $c_{bad} = P_{n-2}(a_0, \dots, a_{n-2}, a_{n-1})$. It is clear that if we consider $c$ to be the opposite bit of $c_{bad}$, there are no elements $a_{i}$ which extend this Long Choice sequence with $P_{n-2}(a_0, \dots, a_{n-2}, a_{i}) = c$. Thus, we can return $a_0, \dots, a_{n-1}$ and $c$ and we are done. 
% \end{proof}

% We remark that in the problem statement of Short Choice, we are explicitly given the initial element $a_0$. However, the above construction holds for any arbitrary $a_0$. Thus, as we did with Long Choice, we can consider a variant of Short Choice (call it Short Choice with no initial element) where we are simply given the predicate functions and no initial element. This problem must also be total. Using the same arguments as in the case of Long Choice, we can argue that the two variants of the Short Choice problem are equivalent. 

%We can now argue that Short Choice is PEPP-hard.

\begin{theorem}
   {\sc  Short Choice} is PEPP-hard
\end{theorem}

% \begin{proof}
%     Consider a PEPP-complete problem, Empty, which is given by a poly(n)-sized circuit $C$: 
    
%     $$C: [2^n-2] \mapsto [2^n-1] $$
    
%     where the challenge is to find an element, $e\in{[2^n-1]}$ such that for all $i\in{[2^n - 2]}$, $C(i) \neq {e}$. 
    
%     % We first redefine the circuit $C$. We define $d_1 := C(1)$, and pick any value, $d_2$ in the set $[2^n]$ which is not equal to $d_1$. We define a new circuit $C'$ with the following domain and range:
    
%     % $$C' : [2^n - 1]\setminus{1} \mapsto [2^n]\setminus{d_1} $$
    
%     % Note that we have excluded $1$ from the domain of $C'$, and $d_1$ from the range of $C'$. Now, on input $i$, the circuit $C'$ has the following behavior:
%     % \begin{enumerate}
%     %     \item $C'(i) = d_2$ if $C(i) = d_1$. 
%     %     \item $C'(i) = C(i)$ otherwise
%     % \end{enumerate}
    
%     % The challenge with this circuit remains the same as with Empty: find an element of the range which does not belong to the image of $C'$. To prove that such an element must exist, there are two cases to consider. First, suppose the input $1$ is the only element which $C$ maps to $d_1$. Then, $C'$ behaves exactly the same as $C$ on all inputs (excluding $1$). Therefore, there must exist an element of $[2^n]\setminus{d_1}$ which does not belong to the image of $C'$. In the second case, suppose there is more than one distinct input which $C$ maps to $d_1$. Then, there must be at least two distinct elements in $[2^n]$ which do not belong to the image of $C$. The image of $C'$ has at most one more element than the image of $C$: $d_2$. Since there are at least two elements in $[2^n]\setminus{d_1}$ which are not in the image of $C$, there must be at least one element of this set which is not in the image of $C'$. Conversely, consider any element of $[2^n]\setminus{d_1}$ which is not in the image of $C'$. This element is also not part of the image of $C$ (based on the above definition of $C'$). 
    
%     % Thus, to solve the $PEPP$ problem, it suffices to find an element of the $2^n - 1$ element set $[2^n]\setminus{d_1}$ which is not in the image of $C'$.
    
%     % Note that $C$ defines a mapping of $2^n - 2$ elements to a set of $2^n - 1$ elements. 
    
%     We now define a Short Choice problem whose solution allows us to recover a solution to this problem.
    
%     The universe, $U$, of this problem consists of the elements in the set $[2^n - 2]$ (the domain of $C$). It now suffices to define a sequence of predicate functions, $P_0, \dots, P_{n-2}$. 

%     Each predicate function $P_i$ takes as input the distinct elements $a_0, a_1, \dots, a_i, a_{j}$ and follows a similar procedure. First, it calculates a set $H_i$ of elements belonging to the range of $C$. This set $H_i$ has the form $[x_i, y_i]\setminus \{C(a_0), C(a_1), \dots, C(a_i) \}$. $P_i$ then calculates the \textbf{midpoint} of $H_i$, defined as the smallest value $k\in{H_i}$ such that half of the elements of $H_i$ are less than or equal to $k$. $P_i$ returns $1$ if $C(a_j)$ is less than or equal to the midpoint of $H_i$ and $0$ otherwise.
    
%     It now remains to define the sets $H_i$. The sets $H_i$ are defined inductively with the following two key properties:
    
%     \begin{enumerate}
%         \item $|H_i| \geq 2^{n-i} - 2$
%         \item If $a_0, a_1, \dots, a_i$ is a Long Choice subcertificate, then for every $k \in \{0, 1, \dots, i-1 \}$, $C(a_j)\in H_{k} \bigcup \{C(a_0), C(a_1), C(a_2), \dots, C(a_k) \}$ whenever $j > k$. 
%     \end{enumerate}
    
%     As a base case, given a first input of $a_0$, $P_0$ defines $H_0 := [2^n - 1] \setminus \{ C(a_0) \}$. This satisfies the first inductive property: $[2^n - 1] \setminus \{ C(a_0) \}$ has $2^{n-0} - 2$ elements. 
    
%     To see why $H_0$ satisfies the second inductive property, note that $H_0 \bigcup C(a_0)$ is actually the set $[2^n - 1]$ - the range of $C$! Therefore, for any Long Choice subcertificate, $a_0, a_1, \dots, a_i$, we will have, for all $k \in \{1, \dots, i\}$, that $C(a_k) \in H_0 \bigcup C(a_0)$, as desired. 


%     Now, suppose that the $H_0, \dots, H_i$ have been defined in such a way that they satisfy the two inductive properties. Suppose $P_i$ takes as input a valid Long Choice subcertificate $a_0, \dots, a_i$, along with a final element $a_{i+1}$. Then, $P_i$ first uses the elements $a_0, \dots, a_i$ to define $H_i$. Next, it calculates the midpoint of $H_i$. Then, $P_i(a_0, a_1, \dots, a_i, a_{i+1})$ returns $1$ if $C(a_{i+1})$ is less than or equal to the midpoint and $0$ otherwise. Accordingly, we define $H_{i+1}$ as follows:
%     \begin{enumerate}
%         \item If $P_i(a_0, \dots, a_i, a_{i+1})$ is $1$, then we define $H_{i+1}$ to be the elements of $H_i\setminus{C(a_{i+1})}$ which are less than or equal to the midpoint of $H_i$ 
%         \item Otherwise, we define $H_{i+1}$ to be the elements of $H_i\setminus{C(a_{i+1})}$ which are greater than the midpoint of $H_i$
%     \end{enumerate}
    
%     To prove that the first inductive property holds for $H_{i+1}$, recall that by our inductive assumption, $H_{i}$ contains at least $2^{n-i} - 2$ elements. By definition, the midpoint will split this set into two sets, $A$ and $B$, each of size at least $2^{n-i-1} - 1$. $H_{i+1}$ is defined as either $A \setminus C(a_{i+1})$ or $B \setminus C(a_{i+1})$. Thus, in either case, $H_i$ has at least $2^{n-i-i} - 2$ elements, as desired. 
    
%     To prove that the second property holds, assume without loss of generality that $C(a_i)$ is greater than the midpoint of $H_{i-1}$. Then, as described above, we define $H_i$ to be the subset of $H_{i-1}\setminus C(a_i)$ containing elements greater than the midpoint of $H_{i-1}$. 
    
%     Now, in order for $P_{i-1}(a_0, a_1, \dots, a_{i-1}, a_j)$ to be constant for all $j \geq i$, we must have that $C(a_j)$ is also greater than the midpoint of $H_{i-1}$. However, by the second inductive assumption, we know that $C(a_j)$ must belong to $H_{i-1} \bigcup \{C(a_0), \dots, C(a_{i-1}) \}$. If we apply these two facts together, we conclude that $C(a_{j})$ must belong to the set $H_{i} \bigcup \{a_0, \dots, a_{i-1}, a_i \}$. Letting $j = i+1$ in our case proves that the second inductive property holds.

%     Finally, consider any certificate to this instance. It consists of a Long Choice subcertificate $a_0, \dots, a_j$ ($j \leq n-2$) and a bit, $c$. As we know, this bit $c$ has the following property: there is no node $a_{j+1}$ which both extends the certificate and also has $P_{j}(a_0, \dots, a_{j}, a_{j+1}) = c$. 
    
%     Consider the set $H_{j}$; it has size at least $2^{n - (j-2)} - 2 \geq 2^{n - (n-2)} - 2 = 2$. Thus, the midpoint of $H_{j}$ splits $H_{j}$ into two nonempty subsets of size at least $1$. Let $A$ denote the subset of $H_{j}$ containing elements less than or equal to its midpoint, and let $B$ denote the subset of $H_{j}$ containing elements greater than its midpoint. Suppose that $c = 0$. Then we can conclude that there are no elements $C(a_{j+1}) \in B$. If there were, we could pick such an element to extend the Long Choice sequence. Thus any element of $B$ would be a solution to our problem. Similarly, if $c = 1$; then we can similarly conclude that there are no elements $C(a_{j+1}) \in A$; thus any element of $A$ would be a solution to our problem. Finally, note that we can easily identify which elements belong to the set $A$ and $B$; as mentioned earlier, they take the form $[x_i, y_i]\setminus \{C(a_0), C(a_1), \dots, C(a_i) \}$. This completes the proof. 
% \end{proof}

We can define the class PSC (Polynomial Short Choice) to be the class whose complete problem is {\sc Short Choice}. 

%Since PEPP is contained in PSC, we must ask: do there exist problems which are unlikely to belong to PEPP but do belong to PSC? 

% \subsection{Large Tournament Dominating Set} 
% Papadimitriou and Yannakakis introduced the classes LOGNP and LOGSNP in \cite{Papadimitriou1996LogNP}. In these classes, the problem, Tournament Dominating Set, encapsulates the following phenomenon: given a tournament between $n$ individuals, there must exist a dominating set of size at most $log(n)$.  

% Here, we define a generalization of this problem using concisely represented circuits: 

% \begin{defi}[Problem: Large Tournament Dominating Set]
% We are given a poly(n)-sized circuit, $C$: 

% $$C: \{0, 1 \}^n \mapsto \{0, 1\} $$

% $C$ defines a tournament of $2^n$ players; each player is represented by a $n$-bit string in $\{0, 1\}^n$. For two players whose $n$-bit representations are $x$ and $y$ ($x < y$), we say:

% \begin{enumerate}
%     \item $x$ defeats $y$ if $P(x, y) = 1$.
%     \item $y$ defeats $x$ if $P(x, y) = 0$. 
% \end{enumerate}

% The problem is to find a collection, $A$, of at most $n$ distinct players $a_0, a_1, \dots, a_{n-1}$ with the property that no player in the tournament defeats all players in $A$.
% \end{defi}

% The proof of totality follows a simple halving argument described in \cite{Papadimitriou1996LogNP}; we provide a brief sketch here:
% \begin{proof}
%     Let $S_0$ denote the set of all players in the tournament. The total number of games played is $${2^n\choose{2}} = \frac{2^n*(2^n - 1)}{2}$$. In each game, there is one winner and one loser. Therefore, there are $\frac{2^n*(2^n - 1)}{2}$ total victories. Let $k$ be the average number of victories by each individual player over the course of the entire tournament. We know that $k = \frac{2^n*(2^n - 1)}{2} * \frac{1}{2^n} = \frac{2^n-1}{2}$. Therefore, there must exist an element which has at least $\frac{2^n-1}{2}$ victories; in other words, such a player must defeat at least half of the opponents. Denote this player by $a_0$ and consider the set of players which defeat $a_0$; call this set $S_1\subset{S_0}$. Furthermore, consider the "subtournament" given by all the games played between players who belong to the set $S_1$. We can use the argument above to conclude there must exist a player, $a_1\in{S_1}$ who defeats at least half of the elements in $S_1$. We can define $S_2\subset S_1$ to be the set of players who defeat $a_1$ and continue this procedure. Note that as we continue this procedure, the sets $S_i$ are guaranteed to approximately \textit{halve} in size: $|S_i| \leq |S_{i-1}/2|$. Since $|S_0| = 2^n$, this construction can only continue for at most $n$ steps. Furthermore, if some set $S_k$ has size $0$, this, by definition, implies that there is no player in the tournament which defeats all of the following players: $a_0, a_1, \dots, a_k$.
% \end{proof}

% Unfortunately, this problem does not seem to cleanly belong to Short Choice (or PEPP, for that matter). However, we can introduce a related problem which is equivalent to Large Tournament Dominating Set. We first introduce some machinery. 

% \begin{defi}[Binary Antisymmetric Predicate]
% A \textbf{binary antisymmetric predicate} is a binary function, $P$ with the property that for any distinct inputs, $a$ and $b$, 

% $$P(a, b) = \neg P(b, a)$$
% \end{defi}

% Consider a universe of objects, $U = \{0, 1\}^n$. A binary antisymmetric predicate function, $P$: 

% $$P : U^2 \mapsto \{0, 1\}$$

% defines a tournament on the graph $U$. Specifically, for any distinct elements $a$ and $b$, we say $P(a, b)$ outputs $1$ if $a$ defeated $b$ and $0$ otherwise. Note the importance of symmetry here; we can equivalently consider $P(b, a)$ to determine whether $b$ defeated $a$ or lost to $a$. 

% \begin{defi}[Problem: Binary Antisymmetric Short Choice]
%     We are given a universe, $U$, consisting of the set of $n$-bit binary strings: $\{0, 1\}^n$. We given a binary antisymmetric predicate function, defined on this universe: 
    
%     $$P: U^2 \mapsto \{0, 1\} $$
    
%     The problem is to find a sequence of distinct nodes $a_0, a_1, \dots, a_k$ ($k \leq {n}$ with the following two properties: 
    
%     \begin{enumerate}
%         \item $P(a_i, a_j) = 0$ for all $i < j$. 
%         \item The sequence cannot be extended with an element $a_{k+1}$ in such a way that it still satisfies property $1$. 
%     \end{enumerate}
% \begin{defi}

% \begin{theorem}
%     Binary Antisymmetric Short Choice is a total problem.
% \end{theorem}

% \begin{proof}
%     First note that the binary antisymmetric predicate function defines a tournament on the set, $U$ (as explained above). We can then use the argument from the proof of totality for Large Tournament Dominating Set to construct the sequence $a_0, a_1, \dots, a_k$. There must exist a node, $a_0$ that defeats half of the other nodes in the universe. We then consider the nodes that \textit{defeat} $a_0$ and apply this logic again. (See the proof of totality for Large Tournament Dominating Set for the complete argument). Note that any node $a_i$ which defeats $a_0$ has $P(a_0, a_i) = 0$. If we continue the procedure, we will by, definition, construct a sequence $a_0, \dots, a_k$ ($k \leq n$) that satisfies property $1$. Furthermore, when we finish this construction, we will arrive at a dominating set, which means there are no other elements which defeats each of $a_0, \dots, a_k$. This, in turn means, the sequence cannot be extended. 
% \end{proof}

% It is clear that Binary Antisymmetic Short Choice and Large Tournament Dominating Set are equivalent (we can simply let the predicate function, $P$ in the former problem be equal to the circuit, $C$, in the latter problem). 

% \begin{theorem}
%     Binary Antisymmetic Short Choice is equivalent to Large Tournament Dominating Set.
% \end{theorem}

% Note that we can generalize the idea of an antisymmetric predicate function to cases of arbitrary arity. For example, we can define a 3-ary predicate function $P(a, b, c)$ with the property that for any input $a$, $P(a, b, c) = \neg P(a, c, b)$. This can allow us to define a generalized Antisymmetric Short Choice problem.

% So far, we have formulated many problems quantified by predicate functions. If we give the predicate functions certain properties (for example, make them binary and antisymmetric) we can characterize problems whose proof of totality is based on extremal combinatorics. 

% Some things to further explore...
% \begin{enumerate}
%     \item We can consider binary antisymmetric Long Choice - this is equivalent to Ramsey!
%     \item There are other problems from the LOGNP paper which we can perhaps place into one of these complexity classes...
% \end{enumerate}



==> Sunflower.tex <==
\section{Sunflowers}
An important aspect in extremal combinatorics is the extremal \textit{bound}: how large a system has to be to guarantee that the desired combinatorial structure exists. Often times, the tightest bounds are unknown - improving these bounds is an important research tradition in Combinatorics \citep{Alweiss2020} \citep{ConlonFerber2020}. 

However, despite this uncertainty, we can still use weaker extremal bounds to define provably hard TFNP search problems, which we can then relate to the subclasses of TFNP. In this section, we focus on the Sunflower Lemma \citep{jukna}, but this paradigm for reasoning about extremal problems can be applied to many other problems as well.


% a more specialized proof often leads to substantial improvements in extremal bounds. See \citep{Alweiss2020} for one such example. In this section, we demonstrate that despite  

% We refer the reader to \citep{jukna} for a more complete discussion of the Sunflower Lemma. 

We begin with some basic definitions.

\begin{defi}
	A {\em $k$-set system} is a collection of distinct sets in which every set contains exactly $k$ elements. A collection of distinct sets $S_1, \dots, S_n$ is a {\em sunflower} if for all $i$, $j$, $S_i \cap {S_j}$ is the same.
\end{defi}

The Sunflower lemma states that for all positive integers $k, s$, there is a number $f(k,s)$ such that every $k$-set system of size $f(k,s)$ contains a sunflower of size $s$. The lemma was formulated and proved by Erd\H{o}s and Rado \cite{ErdosRadoSunflower} for $f(k,s)=k!(s-1)^{k+1}$, using an inductive proof that applies an iterative pigeonhole argument.
The conjecture is that $f(k,s) \leq C^k$ for some constant C that depends only on $s$. Progress on improving the upper bound on $f(k,s)$ was made recently in \cite{Alweiss2020}.


%\begin{theorem}
%	\textbf{Sunflower Lemma: } We are given a $k$-set system, $F$, of size $k! * s^{k+1}$. There exists a sunflower of size $s+1$. 
%\end{theorem}

% The sunflower lemma can be formulated as a problem in TFNP, as long as we note that 
% $$ n! * n^{n+1} \leq{n^n * n^n} = 2^{2nlogn}$$

A computational problem based on the Sunflower Lemma was formulated in \citep{Komargodski2019},
and shown to be hard on average assuming the existence of collision resistant hash function.
Here, we use an even weaker bound to define a problem which we call {\sc Naive Sunflower}, and relate it to the multi-color Ramsey problem.

\begin{defi}[{\sc Naive Sunflower}]
	We are given a poly($k$)-sized circuit 
	$$C: \{0,1\}^{k^3 \log k} \mapsto (\{0,1\}^{k^3 \log k})^k $$
	which is supposed to specify a family of $2^{k^3 \log k}$ distinct sets of size $k$ over a universe of $2^{k^3 \log k}$ elements
	(each element is represented by
	 a $k^3 \log k$-bit string).   The problem is to find either: 
	\begin{enumerate}
		\item (An error): An index $i$ such that the set (represented  by) $C(i)$ contains two identical elements, or find two distinct indices $i$, $j$ such that the sets $C(i), C(j)$ are equal,or
		\item A sunflower of size $k^2$.
	\end{enumerate}
\end{defi}

Following the exact same argument presented in \citep{Komargodski2019}, this problem is hard on average assuming that Collision Resistant Hash Function families exist. 



% \begin{defi}[Problem Statement: Sunflower]
% 	We are given a poly(n)-sized circuit 
% 	$$C: \{0,1\}^{2nlogn} \mapsto (\{0,1\}^n)^n $$
	
% 	which maps $2nlogn$-bit strings into sets of $n$ different $n$-bit strings. It implicitly defines an $n$-set system of size $n^{2n}$.  The challenge is to find either: 
% 	\begin{enumerate}
% 		\item Two distinct indices $i_1$, $i_2$ with $C(i_1) = C(i_2)$. Here, we define equality as set equality. Namely, that the set $C(i_1)$ is equal to the set $C_{i_2}$. 
% 		\item A sunflower of size $n+1$. That is, $n+1$ distinct indices, $i_1, \dots, i_{n+1}$ such that $C(i_1), \dots, C_{n+1}$ forms a sunflower. 
% 		\item (An error): An index $i_1$ such that $C(i_1)$ contains two identical $n$-bit strings. Such an error means that $C_{i_1}$ is not a valid set. 
% 	\end{enumerate}
	
% \end{defi}


% \subsection{Understanding the Relation between PPP, Sunflower, Ramsey, and Long Choice} 

% It seems that the finitary pigeonhole principle provides a (naive) quantitative bound in the proof of the sunflower lemma. These bounds are not necessarily optimal. Recent work by \citep{Alweiss2020} has shown that fewer sets are required to guarantee the existence of a sunflower. \citep{rao2020} has also proved a similar bound. 

% Nevertheless, as explained in \citep{Komargodski2019}, it is clear that even though the Sunflower TFNP problem as defined above has a suboptimal extremal bound, it is still a hard problem under standard cryptographic hardness assumptions.  

% The proof of the finitary sunflower lemma uses a specialized version of the pigeonhole principle. In particular, the proof uses the following argument repetitively: either there are $n+1$ disjoint sets, or by the pigeonhole principle, there are a large number of sets containing one element, $e_i$ in common. We can modify the above sunflower problem to have a weaker extremal bound which makes the problem directly compatible with Ramsey and Long Choice. 

% From a computational perspective, it is unclear how to find this maximally disjoint set. This is why it is difficult to reduce that problem to Long Choice; the bound of $2^{2nlogn}$ assumes that this element $e_i$ can be defined by $log(n)$ (as opposed to $n$ constraints).

% There are two key differences between the original Sunflower problem statement and this one. First, the universe of elements is larger. The reason for this modification is to avoid a situation in which our set system is guaranteed to have repeated elements by a pigeonhole argument. Second, our system now contains $2^{n^3log(n)}$ sets.

% Following the exact argument presented in \citep{Komargodski2019}, can make two observations about the hardness of the Naive Sunflower problem. Firstt, it is also hard under the assumption that Collision Resistant Hash Functions exist. Second, it is also PWPP-hard. 

% However, unlike the sunflower problem presented in \citep{Komargodski2019}, Naive Sunflower is guaranteed to have sunflowers of size greater than $n$. In fact, it is guaranteed to have sunflowers of size greater than $n^2$. 

We will reduce {\sc Naive Sunflower} to Multi-color Ramsey by using a characterization of large sunflowers as a pairwise equidistant collection of points in a metric space. Given a $k$-set system $F$, define the distance $d(A,B)$ between any two sets $A, B$ of $F$ as $d(A,B) = |A \Delta B|/2$, where $A \Delta B = \{A\setminus{B} \}\cup \{B\setminus{A}\}$ is their symmetric difference
(it has even size since $A, B$ have the same size).
The function $d$ is a valid metric.
Clearly, any sunflower in $F$ is a set of pairwise equidistant points in this metric.

Conversely, by a result of Deza \citep{DezaEquidistant}, any collection of at least $k^2-k+2$ pairwise equidistant $k$-sets must form a sunflower. Therefore, in this regime, we can reduce the problem of finding a sunflower of size $k^2$ to the problem of finding $k^2$ pairwise equidistant sets. In turn, we can reduce this problem to the multi-color Ramsey problem.

\begin{theorem}
    {\sc Naive Sunflower} reduces to {\sc $(\sqrt{n},n)$-Ramsey}.
\end{theorem}

\begin{proof}
    Consider an instance of {\sc Naive Sunflower}, given by a circuit $C$. As above, $C$ is supposed to define a set system consisting of $2^{k^3 \log k}$ sets, where each set contains $k$ elements. The core idea behind our reduction is simple: we construct a graph consisting of $2^{k^3 \log k}$ nodes, where the $i$-th node $u_i$ corresponds to the set $C(i)$. To color the edges of this graph, we use $k$ colors, given by the numbers $1, 2, \dots, k$. Every edge $(u_i,u_j)$ is colored as follows. If $C(i), C(j)$  are distinct $k$-sets, then assign color $d(C(i),C(j))$ to the edge $(u_i,u_j)$.
    If one of $C(i), C(j)$ is not a $k$-set, e.g. contains a duplicate element, or if the sets are equal, then assign color 1 to the edge $(u_i,u_j)$.
    
    Let $n = k^2$. Since the graph has 
    $2^{k^3 \log k} = k^{nk}$ nodes, it contains a monochromatic clique of size $n = k^2$
    by Ramsey's Theorem. Let $M$ be any such monochromatic clique of size $k^2$.
    If $M$ contains a node $u_i$ such that $C(i)$ is not a $k$-set, or if it contains two nodes $u_i, u_j$ such that $C(i), C(j)$ are equal sets, then we have a violation for the circuit $C$.
    Otherwise, the collection $\{ C(i) | u_i \in M \}$ has $k^2$ pairwise equidistant sets, and thus by Deza's theorem, they form a sunflower.
\end{proof}

We have shown earlier that {\sc ($r,n$)-Ramsey} is in PLC for any $r,n $; thus we can conclude: 

\begin{corollary}
    {\sc Naive Sunflower} is in PLC.
\end{corollary}






